TAX-Pose: Task-Specific Cross-Pose Estimation for Robot Manipulation

How do we imbue robots with the ability to efficiently manipulate unseen objects and transfer relevant skills based on demonstrations? End-to-end learning methods often fail to generalize to novel objects or unseen configurations. Instead, we focus on the task-specific pose relationship between relevant parts of interacting objects. We conjecture that this relationship is a generalizable notion of a manipulation task that can transfer to new objects in the same category; examples include the relationship between the pose of a pan relative to an oven or the pose of a mug relative to a mug rack. We call this task-specific pose relationship "cross-pose" and provide a mathematical definition of this concept. We propose a vision-based system that learns to estimate the cross-pose between two objects for a given manipulation task using learned cross-object correspondences. The estimated cross-pose is then used to guide a downstream motion planner to manipulate the objects into the desired pose relationship (placing a pan into the oven or the mug onto the mug rack). We demonstrate our method's capability to generalize to unseen objects, in some cases after training on only 10 demonstrations in the real world. Results show that our system achieves state-of-the-art performance in both simulated and real-world experiments across a number of tasks. Supplementary information and videos can be found at https://sites.google.com/view/tax-pose/home.

==> figures/half_width_corl_explanation.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/corl-explanation-v7.pdf}
    \caption{Visualization of the properties of cross-pose.  If we transform both the action (mug) and the anchor (rack) objects by the same transform, then the relative pose between these objects is unchanged (the mug is still ``on" the rack) so the cross-pose is unchanged.}
    \label{cross_pose}
\end{wrapfigure}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> main_old_ref_not_right.tex <==
% \documentclass{article}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % When it's time to create a version which has 
% % an appendix attached, just do \appendixtrue
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newif\ifappendix
% \appendixfalse
% %%%%%%%%%%%%%%%%%
% % Controls whether references get imported.
% %%%%%%%%%%%%%%%%%
% \ifappendix
%   % using appendix
% \else
%     \input{_external_deps.tex}
%     \myexternaldocument{appendix}
% \fi

% \usepackage[final]{corl_2022}
% %\usepackage{corl_2022} % Use this for the initial submission.
% \usepackage{times}

% % numbers option provides compact numerical references in the text. 
% \usepackage[numbers]{natbib}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{wrapfig}
% \usepackage{adjustbox}
% \usepackage{floatrow}
% % Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \usepackage{blindtext}
% \usepackage{etoc} 
% \usepackage{bibunits}

% \renewcommand{\contentsname}{Appendix}



% \input{math_definitions.tex}


% \usepackage{blindtext}
% \usepackage{enumitem,kantlipsum}
% \usepackage[font={footnotesize}]{caption}
% \usepackage{color, soul} % This allows us to highlight text that you want your co-authors to review
% % \renewcommand\hl[1]{#1} % Uncomment this to turn off highlighting
% % use \hl{text} to highlight something
% \input{preamble.tex}
% \newcommand{\rebuttal}[1]{{\color{magenta} #1}}
% \newcommand{\cameraready}[1]{{\color{blue} #1}}
% %\title{TS-CorrNet: Learning Task-Specific Point Cloud Correspondence }
% \title{TAX-Pose: Task-Specific Cross-Pose Estimation\\ for Robot Manipulation}


% \author{
%   Chuer Pan\thanks{Equal Contribution. See Appendix \ref{appendix:contributions} for a detailed list of each author's contributions.}, Brian Okorn\footnotemark[1], Harry Zhang\footnotemark[1], Ben Eisner\footnotemark[1], David Held \\
%   Robotics Institute, School of Computer Science\\
%   Carnegie Mellon University, 
%   United States\\
%   \texttt{\{chuerp, bokorn, haolunz, baeisner, dheld\}@andrew.cmu.edu} \\

% % \thanks{Contribution List}

% }
% \begin{document}
% \maketitle

% %===============================================================================

% \begin{abstract}
%    How do we imbue robots with the ability to efficiently manipulate unseen objects and transfer relevant skills based on demonstrations? End-to-end learning methods often fail to generalize to novel objects or unseen configurations. Instead, we focus on the task-specific pose relationship between relevant parts of interacting objects. We conjecture that this relationship is a generalizable notion of a manipulation task that can transfer to new objects in the same category; examples include the relationship between the pose of a pan relative to an oven or the pose of a mug relative to a mug rack. We call this task-specific pose relationship ``cross-pose" and provide a mathematical definition of this concept. We 
%    propose a vision-based system that learns to estimate the cross-pose between two objects for a given manipulation task using learned cross-object correspondences. The estimated cross-pose is then used to guide a downstream motion planner to manipulate the objects into the desired pose relationship (placing a pan into the oven or the mug onto the mug rack). 
%    %We train a cross-pose estimator in simulation and we demonstrate the capability of our system to generalize to unseen objects in both simulation and the real world, deploying our policy on a Franka Emika with no finetuning.
%    We demonstrate our method's capability to generalize to unseen objects,
%    in some cases after training on only 10 demonstrations in the real world.
%    %deploying our policy on a Franka Panda 
%    Results show that our system achieves state-of-the-art performance in both simulated and real-world experiments across a number of tasks. Supplementary information and videos can be found on our \href{https://sites.google.com/view/tax-pose/home}{project website}.
% \end{abstract}

% % Two or three meaningful keywords should be added here
% \keywords{Learning from Demonstration, Manipulation, 3D Learning} 

% \maketitle
% \begin{figure*}[h]
%     \centering
%     % \includegraphics[width=\textwidth, trim={100 210 175 220}, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-NoBack.pdf}
%     % \includegraphics[width=\textwidth, trim={230 210 290 220}, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-4.pdf}
%     \includegraphics[width=\textwidth, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-5-NoBack2.pdf}
%     \vspace{-20pt}
%     \caption{To solve a relative placement task, TAX-Pose uses cross-object attention to estimate dense cross-object correspondences and importance weights for each object point. This dense estimate is mapped to a single ``cross-pose" which the robot uses to accomplish the given task.}
%     \label{fig:teaser_pipeline}
% \end{figure*}
% \section{Introduction}
% \input{sec-1-intro}
% \section{Related Work}
% \input{sec-2-rw}
% \input{sec-3-ps}
% \section{Method}
% % \input{sec-4-methods}
% \input{sec-4-methods-2}
% \section{Experiments}
% \input{sec-5-exps}
% \section{Conclusion and Limitations}
% \input{sec-6-conclusion}

% \bibliography{ref}  % .bib

% \begin{bibunit}[corlabbrvnat]
% \appendix
% \input{appendix}
% \putbib[ref]
% \end{bibunit}
% \end{document}


==> tables/ablation-in-main.tex <==
% \begin{table}[ht]
% \begin{varwidth}[b]{0.1\linewidth}
%     \centering
%       \renewcommand{\arraystretch}{1}
%     %  \resizebox{6\linewidth}{!}{
%     \begin{tabular}{c|c c c}
%     % \hline
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%  % }
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \qquad
% \begin{varwidth}[b]{}
%     \centering
%       
%      
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%      
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%



% \end{table}


% \begin{table}[htb]
    \begin{minipage}[t]{.3\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        }
        \captionof{table}{ \# Demos vs. Overall Success}

    \end{minipage}%
    \hfill
    \begin{minipage}[t]{.4\textwidth}
        % \small
        \centering
        \label{tab:mug_rack_ablation}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c| c c c}
    \hline
  \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
        % \textit{Loss}&&&\\
          No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
          No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
           No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
            Scaled Combination: 
            %of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ (
            $ 1.1\mathcal{L}_\mathrm{cons} + \mathcal{L}_\mathrm{corr}$ &  0.10 & 0.01 & 0.01 \\
         \hline 
          No Adjustment via Correspondence Residuals  & 0.97 &0.96 & 0.93\\
         \hline 
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
        \hline 
         No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
         No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         \hline 
         3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
        \hline
        Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
        \hline
        \hline
        \textbf{TAX-Pose (Ours)}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
    \hline
    \end{tabular}
    }
        \captionof{table}{Mug Hanging Ablations Results}

    \end{minipage}%
% \end{table}


==> tables/exec-l2-dist-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.70 & 0.80 & 0.83 & 0.90 & 0.70 & 0.92 & 0.70 & 0.86 & 0.73 & 0.74 & 0.66 & 0.87 & 0.74 & 0.69 & 0.63 & 0.67 & 0.63 & 0.75 & 0.72 & 0.83 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.57 & 0.70 & 0.79 & 0.82 & 0.66 & 0.65 & 0.63 & 0.62 & 0.49 & 0.66 & 0.64 & 0.67 & 0.50 & 0.85 & 0.54 & 0.75 & 0.43 & 0.70 & 0.45 & 0.61 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.26 & 0.50 & 0.46 & 0.50 & 0.16 & 0.38 & 0.19 & 0.48 & 0.30 & 0.50 & 0.13 & 0.55 & 0.28 & 0.57 & 0.44 & 0.50 & 0.14 & 0.63 & 0.24 & 0.40 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.14 & 0.68 & 0.16 & 0.69 & 0.10 & 0.73 & 0.10 & 0.84 & 0.17 & 0.76 & \textbf{0.05} & 0.88 & 0.12 & 0.51 & 0.29 & 0.54 & 0.12 & 0.68 & 0.16 & 0.47 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.11} & \textbf{0.10} &\textbf{ 0.12 }& \textbf{0.09} & \textbf{0.02} & \textbf{0.04} & \textbf{0.06} & \textbf{0.08} & \textbf{0.15} & \textbf{0.11} & 0.05 & \textbf{0.05} & \textbf{0.12} & \textbf{0.08} & \textbf{0.28} & \textbf{0.26} & \textbf{0.10 }& \textbf{0.09} & \textbf{0.07} & \textbf{0.06} \\ \hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> tables/exec-l2-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.70&	0.83&	0.70&	0.70&	0.73&	0.66&	0.74&	0.63&	0.63&	0.72\\
Goal-Cond E2E DAgger&0.61&0.79&0.66&0.63&0.49&0.64&0.80&0.64&0.43&0.45\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.26&0.46&0.16&0.19&0.30&0.13&0.28&0.44&0.14&0.24\\
% {Ours w/ Lear}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
{Goal-Cond Goal Flow}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.11&0.12&0.02&0.06&0.15&0.05&0.12&0.28&0.10&0.07\\
\hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> tables/exec-sr-rate-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.02 & 0.01 & 0.03 & 0.00 & 0.10 & 0.05 & 0.03 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.03 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.15 & 0.13 & 0.03 & 0.03 & 0.63 & 0.60 & 0.13 & 0.13 & 0.03 & 0.00 & 0.25 & 0.25 & 0.10 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.15 & 0.15 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.64 & 0.05 & 0.73 & 0.00 & 0.75 & 0.10 & 0.73 & 0.00 & 0.50 & 0.00 & 0.80 & 0.00 & \textbf{0.65} & 0.10 & 0.35 & 0.10 & 0.70 & 0.10 & 0.55 & 0.05 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.78} & \textbf{0.81} & \textbf{0.78} & \textbf{0.78} & \textbf{0.98} & \textbf{1.00} & \textbf{0.88} & \textbf{1.00} & \textbf{0.70} & \textbf{0.73} & \textbf{1.00} & \textbf{1.00} & 0.65 & \textbf{0.65} & \textbf{0.55} & \textbf{0.45} & \textbf{0.73} & \textbf{0.88} & \textbf{0.80} & \textbf{0.80} \\ \hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> tables/exec-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.02&	0.03&	0.10&	0.03&	0.00&	0.00&	0.00&	0.00&	0.00&	0.00\\
Goal-Cond E2E DAgger&0.03&0.00&0.10&0.10&0.00&0.00&0.00&0.00&0.03&0.00\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.15&0.025&0.63&0.13&0.03&0.25&0.10&0.00&0.05&0.15\\
{Goal-Cond Goal Flow}&0.60&0.63&0.73&0.73&0.48&0.85&0.65&0.37&0.48&0.50\\
% \textbf{Ours 2/ FCL Collision Checker}&0.68&0.78&0.77&0.75&0.55&0.93&0.75&0.35&0.70&0.55\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.78&0.78&0.98&0.88&0.70&1.00&0.65&0.55&0.73&0.80\\
\hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> tables/gi-Rt-error.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \setlength\tabcolsep{.2em}
% \begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 40.45 & 0.75 & 37.82 & 0.82 & 38.17 & 0.81 & 37.15 & 0.65 & 44.84 & 0.68 & 32.52 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
% \multicolumn{1}{|l|}{} & E2E DAgger & 36.85 & 0.71 & 34.15 & 0.76 & 36.50 & 0.74 & 36.61 & 0.66 & 40.91 & 0.65 & 30.67 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 35.37 & 0.66 & 31.24 & 0.82 & 33.89 & 0.69 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
% \multicolumn{1}{|l|}{} & Goal Flow & 26.46 & 0.16 & 25.88 & 0.15 & 26.29 & 0.10 & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & 0.18 & 20.96 & 0.24 & 29.02 & 0.23 & 22.13 & 0.20 \\
% % \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \hline
% \multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \end{tabular}
% }
% \caption{Goal Inference Rotational and Translational Error Results. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). }
% \label{tab:gi-Rt}
% \end{table}
% \vspace{-25pt}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.26 & 0.73 & 37.82 & 0.82 & 37.15 & 0.65 & 44.84 & 0.68 & 30.69 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 37.96 & 0.69 & 34.15 & 0.76 & 36.61 & 0.66 & 40.91 & 0.65 & 24.87 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.95 & 0.67 & 31.24 & 0.82 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 26.64 & 0.17 & 25.88 & \textbf{0.15} & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & \textbf{0.18} & 20.96 & \textbf{0.24} & 29.02 & 0.23 & 22.13 & 0.20  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.64} & \textbf{0.16} & \textbf{6.85} & 0.16 & \textbf{2.05} & \textbf{0.10} & \textbf{3.87} & \textbf{0.12} & \textbf{4.04} & \textbf{0.08} & \textbf{12.71} & 0.31 & \textbf{6.87} & 0.37 & \textbf{5.89} & \textbf{0.13} & \textbf{14.93} & \textbf{0.18} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$). Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt}
\end{table}
% \vspace{-25pt}

==> tables/gi-chamfer-dist-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> tables/gi-chamfer-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.69&	0.77&	0.71&	0.72&	0.65&	0.70&	0.65&	0.64&	0.68&	0.67\\
Goal-Cond E2E DAgger&0.49&0.71&0.39&0.56&0.43&0.55&0.42&0.42&0.50&0.43\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.25&0.39&0.19&0.28&0.27&0.11&0.26&0.27&0.33&0.18\\
Goal-Cond Goal Flow&0.14&0.10&0.06&0.16&0.15&0.07&0.05&0.24&0.22&0.18\\
Goal-Cond DCP&0.54&0.66&0.47&0.70&0.28&0.45&0.78&0.32&0.67&0.50\\
Goal-Cond DCP Weighted Sum&0.37	&0.56&	0.19&	0.57&	0.35&	0.23&	0.56&	0.28&	0.48&	0.12\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.07&0.05&0.00&0.09&0.19&0.01&0.03&0.14&0.05&0.08\\
\hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> tables/gi-sr-rate-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.09 & 0.03 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.05 & 0.15 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.00 & 0.10 & 0.10 & 0.00 & 0.05 & 0.00 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.31 & 0.05 & 0.00 & 0.30 & 0.50 & 0.03 & 0.23 & 0.03 & 0.33 & 0.03 & 0.50 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.40 & 0.00 & 0.40 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.61 & 0.39 & 0.28 & 0.13 & 0.75 & 0.50 & 0.53 & 0.50 & 0.50 & 0.15 & 0.80 & 0.75 & 0.80 & 0.20 & 0.55 & 0.50 & 0.50 & 0.25 & 0.75 & 0.50 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.74 & 0.42 & 0.75 & 0.40 & 0.88 & 0.63 & 0.78 & 0.22 & \textbf{0.80} & 0.60 & 0.83 & 0.50 & 0.75 & 0.50 & 0.65 & 0.05 & 0.63 & 0.25 & 0.65 & 0.65 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.29 & 0.30 & 0.25 & 0.20 & 0.30 & 0.30 & 0.00 & 0.00 & 0.68 & 0.58 & 0.38 & 0.43 & 0.10 & 0.00 & 0.45 & 0.65 & 0.10 & 0.18 & 0.40 & 0.40 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.38 & 0.44 & 0.20 & 0.20 & 0.65 & 0.63 & 0.05 & 0.15 & 0.45 & 0.60 & 0.58 & 0.38 & 0.15 & 0.50 & 0.45 & 0.35 & 0.28 & 0.20 & 0.65 & 0.65 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.90} & \textbf{0.88} & \textbf{0.93} & \textbf{0.88} & \textbf{1.00} & \textbf{0.98} & \textbf{0.85} & \textbf{0.95} & 0.80 & \textbf{0.70} & \textbf{1.00} & \textbf{1.00 }& \textbf{0.95} & \textbf{0.80} & \textbf{0.75} & \textbf{0.75} & \textbf{0.95 }& \textbf{0.93 }& \textbf{0.90} & \textbf{0.95} \\ \hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> tables/gi-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.09&	0.00&	0.10&	0.00&	0.15&	0.25&	0.15&	0.00&	0.10&	0.05\\
Goal-Cond E2E DAgger&0.31&0.00&0.50&0.23&0.33&0.50&0.25&0.15&0.40&0.40\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.61&0.28&0.75&0.53&0.50&0.80&0.80&0.55&0.50&0.75\\
{Goal-Cond Goal Flow}&0.74&0.75&0.88&0.78&0.80&0.83&0.75&0.65&0.625&0.65\\
Goal-Cond DCP&0.29&0.25&0.30&0.00&0.68&0.38&0.10&0.45&0.10&0.40\\
Goal-Cond DCP Weighted Sum&0.38&	0.20&	0.65&	0.05&	0.45&	0.58&	0.15&	0.45&	0.275&	0.65\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.90&0.93&1.00&0.85&0.80&1.00&0.95&0.75&0.95&0.90\\
\hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> tables/mug_hanging_exp_main.tex <==
    \noindent \begin{minipage}[t]{.4\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        \captionof{table}{ \# Demos vs. Overall Success}

    \end{minipage}%
    \qquad\qquad
    \begin{minipage}[t]{.5\textwidth}
        % \small
        \centering
        \label{tab:mug_resul}
  \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
        \captionof{table}{Mug Hanging Ablations Results}

    \end{minipage}%
    
    \begin{table}[h]
    % \small
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    }
    \caption{Mug on Rack Simulation Task Success Results
    % \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
    }
    \label{tab:mug_on_rack_exp}
\end{table}

==> tables/mug_on_rack_exp.tex <==
\begin{table}[h]
    % \small
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    }
    \caption{Mug on Rack Simulation Task Success Results
    % \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
    }
    \label{tab:mug_on_rack_exp}
\end{table}
% \vspace{-1em}
% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%      & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%     % & Grasp & Place & Overall\\
%     \hline
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
%     \hline
%         \textbf{Upright Pose} & & &\\
%          \hline
%          DON \cite{florence2018dense} & 0.91 &0.50 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88 \\
%          TAX-Pose (Ours) & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%         %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

%     \textbf{Arbitrary Pose} & & & \\
%      \hline
%          DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
%          NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
%           TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug on Rack Simulation Task Success Results
%     \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
%     }
 
%     \label{tab:mug_on_rack_exp}
% \end{table}

==> tables/mug_on_rack_few_shot.tex <==
% \begin{table}[h]
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%       \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
%         \end{adjustbox}
%     %\caption{Mug on Rack Simulation Task Success Results with Varying Number of Demo Used
%     %\dave{Too much whitespace around this table; wrap text around it}
%     %}
 
%     %  \label{tab:mug_on_rack_few_shot}
     
%  \end{subtable}

% % \hfill
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%      \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
     
%     \end{tabular}
%     \end{adjustbox}

 
%   #%\label{tab:mug_rack_ablation}
%  \end{subtable}
%     \caption{Mug on Rack Ablation  Results}
%     \label{tab:mug_rack_ablation}
% \end{table}


%  \begin{table}[h]
 
%     \centering
     
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
        
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
%     % \dave{Too much whitespace around this table; wrap text around it}
%     }
 
%      \label{tab:mug_on_rack_few_shot}
     
%  \end{table}


% \begin{table}[h]
% \begin{varwidth}[b]{0.33\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \begin{varwidth}[b]{0.2\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%

% \end{table}

 
 \begin{wraptable}{r}{8cm}
 
    \centering
     
    \begin{tabular}{c|c c c}
    % \hline
     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
    \hline
          & 1 & 5 & 10\\
         \hline
         DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
         NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
          TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
    \hline
 
    
    \end{tabular}
        
    \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
    % \dave{Too much whitespace around this table; wrap text around it}
    }
 
     \label{tab:mug_on_rack_few_shot}
     
 \end{wraptable}
 

==> tables/mug_rack_ablation.tex <==
% \begin{table}[h]
\begin{table}[]
  \tiny
    \centering
    \begin{tabular}{c|c c c}
    \hline
    \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
         No Residual Correspondence  & 0.97 &0.96 & 0.93\\
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
         3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
         TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
    \hline
    \end{tabular}
    \caption{Mug Hanging Ablations Results}
    \label{tab:mug_rack_ablation}
\end{table}



 

==> tables/rw-placement.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
% \centering
% \begin{tabular}{|r|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\textbf{AVG. SR}} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
% Goal Flow & 0.31 & 0.18 & 0.38 & 0.37 \\ \hline
% \textbf{TAX-Pose} & 0.92 & 0.95 & 0.95 & 0.85 \\ \hline
% \end{tabular}
\begin{tabular}{|r|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
Goal Flow & 0.18 & 0.38 & 0.37 \\ \hline
\textbf{TAX-Pose} & 0.95 & 0.95 & 0.85 \\ \hline
\end{tabular}
\label{rw-placement}
\caption{PartNet-Mobility Objects Placement Task Real-World Results.}
\end{table}

==> tables/single_goal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h]
\begin{subtable}[h]{\textwidth}
    \centering
    \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
    \hline
    \rule{0pt}{2.5em}
    
    & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
    
    & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
    
    \end{tabular}
    \caption{First Week}
    \label{tab:week1}
\end{subtable}
\begin{subtable}[h]{\textwidth}
        \centering
        \begin{tabular}{l | l | l}
        Day & Max Temp & Min Temp \\
        \hline \hline
        Mon & 20 & 13\\
        Tue & 22 & 14\\
        Wed & 23 & 12\\
        Thurs & 25 & 13\\
        Fri & 18 & 7\\
        Sat & 15 & 13\\
        Sun & 20 & 13
       \end{tabular}
      \caption{First Week}
       \label{tab:week2}
\end{subtable}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
% \multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
% \multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
% \multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
% \multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
% \multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
% \end{tabular}
% }
\caption{Ben testing something o}
\label{tab:single-goal}
\end{table}

==> taxpose/_external_deps.tex <==
% Hackily have to compile the appendix.
% copied from: https://www.overleaf.com/learn/how-to/Cross_referencing_with_the_xr_package_in_Overleaf#When_should_I_use_the_xr_package.3F

%----Helper code for dealing with external references----
% (by cyberSingularity at http://tex.stackexchange.com/a/69832/226)

\usepackage{xr}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
\typeout{(#1)}% latexmk will find this if $recorder=0
% however, in that case, it will ignore #1 if it is a .aux or 
% .pdf file etc and it exists! If it doesn't exist, it will appear 
% in the list of dependents regardless)
%
% Write the following if you want it to appear in \listfiles 
% --- although not really necessary and latexmk doesn't use this
%
\@addtofilelist{#1}
%
% latexmk will find this message if #1 doesn't exist (yet)
\IfFileExists{#1}{}{\typeout{No file #1.}}
}\makeatother

\newcommand*{\myexternaldocument}[1]{%
\externaldocument{#1}%
\addFileDependency{#1.tex}%
\addFileDependency{#1.aux}%
}
%------------End of helper code--------------

==> taxpose/figures/half_width_corl_explanation.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/corl-explanation-v7.pdf}
    \caption{Visualization of the properties of cross-pose.  If we transform both the action (mug) and the anchor (rack) objects by the same transform, then the relative pose between these objects is unchanged (the mug is still ``on" the rack) so the cross-pose is unchanged.}
    \label{cross_pose}
\end{wrapfigure}


==> taxpose/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> taxpose/main_old_ref_not_right.tex <==
% \documentclass{article}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % When it's time to create a version which has 
% % an appendix attached, just do \appendixtrue
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newif\ifappendix
% \appendixfalse
% %%%%%%%%%%%%%%%%%
% % Controls whether references get imported.
% %%%%%%%%%%%%%%%%%
% \ifappendix
%   % using appendix
% \else
%     \input{_external_deps.tex}
%     \myexternaldocument{appendix}
% \fi

% \usepackage[final]{corl_2022}
% %\usepackage{corl_2022} % Use this for the initial submission.
% \usepackage{times}

% % numbers option provides compact numerical references in the text. 
% \usepackage[numbers]{natbib}
% \usepackage{caption}
% \usepackage{subcaption}
% \usepackage{wrapfig}
% \usepackage{adjustbox}
% \usepackage{floatrow}
% % Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[][\FBwidth]
% \usepackage{blindtext}
% \usepackage{etoc} 
% \usepackage{bibunits}

% \renewcommand{\contentsname}{Appendix}



% \input{math_definitions.tex}


% \usepackage{blindtext}
% \usepackage{enumitem,kantlipsum}
% \usepackage[font={footnotesize}]{caption}
% \usepackage{color, soul} % This allows us to highlight text that you want your co-authors to review
% % \renewcommand\hl[1]{#1} % Uncomment this to turn off highlighting
% % use \hl{text} to highlight something
% \input{preamble.tex}
% \newcommand{\rebuttal}[1]{{\color{magenta} #1}}
% \newcommand{\cameraready}[1]{{\color{blue} #1}}
% %\title{TS-CorrNet: Learning Task-Specific Point Cloud Correspondence }
% \title{TAX-Pose: Task-Specific Cross-Pose Estimation\\ for Robot Manipulation}


% \author{
%   Chuer Pan\thanks{Equal Contribution. See Appendix \ref{appendix:contributions} for a detailed list of each author's contributions.}, Brian Okorn\footnotemark[1], Harry Zhang\footnotemark[1], Ben Eisner\footnotemark[1], David Held \\
%   Robotics Institute, School of Computer Science\\
%   Carnegie Mellon University, 
%   United States\\
%   \texttt{\{chuerp, bokorn, haolunz, baeisner, dheld\}@andrew.cmu.edu} \\

% % \thanks{Contribution List}

% }
% \begin{document}
% \maketitle

% %===============================================================================

% \begin{abstract}
%    How do we imbue robots with the ability to efficiently manipulate unseen objects and transfer relevant skills based on demonstrations? End-to-end learning methods often fail to generalize to novel objects or unseen configurations. Instead, we focus on the task-specific pose relationship between relevant parts of interacting objects. We conjecture that this relationship is a generalizable notion of a manipulation task that can transfer to new objects in the same category; examples include the relationship between the pose of a pan relative to an oven or the pose of a mug relative to a mug rack. We call this task-specific pose relationship ``cross-pose" and provide a mathematical definition of this concept. We 
%    propose a vision-based system that learns to estimate the cross-pose between two objects for a given manipulation task using learned cross-object correspondences. The estimated cross-pose is then used to guide a downstream motion planner to manipulate the objects into the desired pose relationship (placing a pan into the oven or the mug onto the mug rack). 
%    %We train a cross-pose estimator in simulation and we demonstrate the capability of our system to generalize to unseen objects in both simulation and the real world, deploying our policy on a Franka Emika with no finetuning.
%    We demonstrate our method's capability to generalize to unseen objects,
%    in some cases after training on only 10 demonstrations in the real world.
%    %deploying our policy on a Franka Panda 
%    Results show that our system achieves state-of-the-art performance in both simulated and real-world experiments across a number of tasks. Supplementary information and videos can be found on our \href{https://sites.google.com/view/tax-pose/home}{project website}.
% \end{abstract}

% % Two or three meaningful keywords should be added here
% \keywords{Learning from Demonstration, Manipulation, 3D Learning} 

% \maketitle
% \begin{figure*}[h]
%     \centering
%     % \includegraphics[width=\textwidth, trim={100 210 175 220}, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-NoBack.pdf}
%     % \includegraphics[width=\textwidth, trim={230 210 290 220}, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-4.pdf}
%     \includegraphics[width=\textwidth, clip]{figures/teaser_figures/TAX-Pose-Figures-Pipeline-Robot-5-NoBack2.pdf}
%     \vspace{-20pt}
%     \caption{To solve a relative placement task, TAX-Pose uses cross-object attention to estimate dense cross-object correspondences and importance weights for each object point. This dense estimate is mapped to a single ``cross-pose" which the robot uses to accomplish the given task.}
%     \label{fig:teaser_pipeline}
% \end{figure*}
% \section{Introduction}
% \input{sec-1-intro}
% \section{Related Work}
% \input{sec-2-rw}
% \input{sec-3-ps}
% \section{Method}
% % \input{sec-4-methods}
% \input{sec-4-methods-2}
% \section{Experiments}
% \input{sec-5-exps}
% \section{Conclusion and Limitations}
% \input{sec-6-conclusion}

% \bibliography{ref}  % .bib

% \begin{bibunit}[corlabbrvnat]
% \appendix
% \input{appendix}
% \putbib[ref]
% \end{bibunit}
% \end{document}


==> taxpose/math_definitions.tex <==
\newcommand{\MA}[0]{{\mathcal{A}}}
\newcommand{\MB}[0]{{\mathcal{B}}}

\newcommand{\PA}[0]{\mathbf{P}_{\MA}}
\newcommand{\PB}[0]{\mathbf{P}_{\MB}}
\newcommand{\NA}[0]{N_{\MA}}
\newcommand{\NB}[0]{N_{\MB}}
\newcommand{\TAB}[0]{\mathbf{T}_{\MA \MB}}

\newcommand{\AtoB}[0]{\MA \to \MB}
\newcommand{\BtoA}[0]{\MB \to \MA}

\newcommand{\VA}[0]{\mathbf{\tilde{V}}_{\MA}}
\newcommand{\VB}[0]{\mathbf{\tilde{V}}_{\MB}}


==> taxpose/preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
% \usepackage{hyperref}
\usepackage{multicol}
\usepackage{footmisc}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage[ruled]{algorithm}
\usepackage{bbm}
\usepackage{tablefootnote}
% \usepackage{subcaption}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\useunder{\uline}{\ul}{}
\usepackage[noend]{algorithmic}
% \usepackage[dvipsnames]{xcolor} % load before tikz
\usepackage{tikz}
\usepackage{enumitem}
\usepackage{float}
\usepackage{hyperref}
\usepackage{array}

\usepackage{booktabs} % for professional tables
\usepackage{mathtools}
% \usepackage{subfig}

\usetikzlibrary{math,shapes,positioning}
% \usepackage[font={small}]{caption}
% \usepackage[caption=false, font=footnotesize]{subfig}
\usepackage{listings}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
% Integer range https://tex.stackexchange.com/questions/304662/typesetting-an-integer-interval
\newcommand{\irange}[2]{[#1 \nobreak\mathinner{\ldotp\ldotp}\nobreak #2]}
\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\harry}[1]{{\color{orange}Harry: {#1}}}
\newcommand{\dave}[1]{{\color{red}Dave: {#1}}}
\newcommand{\ben}[1]{{\color{red}Ben: {#1}}}
\newcommand{\brian}[1]{{\color{purple}Brian: {#1}}}
\newcommand{\chuer}[1]{{\color{brown}Chuer: {#1}}}
\newcommand{\clipart}[1]{\includegraphics[height=6mm]{images/#1.png}}


==> taxpose/sec-1-intro.tex <==
 

Many manipulation tasks require a robot to move an object to a location relative to another object.  For example, a cooking robot may need to place a lasagna in an oven, place a pot on a stove, place a plate in a microwave, place a mug onto a mug rack, or place a cup onto a shelf.  Understanding and placing objects in task-specific locations is a key skill for robots operating in human environments. Further, this skill should generalize to novel objects within the training categories, such as placing new trays into the oven or new mugs onto a mug rack.
A common approach in robot learning is to train a policy ``end-to-end," mapping from pixel observations to low-level robot actions.  However, end-to-end trained policies cannot easily reason about complex pose relationships such as the ones described above, and they have difficulty generalizing to unseen object configurations.    



In contrast, we propose 
a method that learns to reason about the 3D geometric relationship between a pair of objects.
For the type of tasks defined above, the robot needs to reason about the relationship between key parts on one object with respect to key parts on another object.  For example, to place a mug on a mug rack, the robot must reason about the relationship between the pose of the mug handle and the pose of the mug rack; if the mug rack changes its pose, then the pose of the mug must change accordingly in order to still be placed on the rack (see Figure~\ref{fig:rel_placement}).  We name this task-specific notion of the pose relationship between a pair of objects as ``cross-pose" and we formally define it mathematically.  Further, we propose a vision system that can efficiently estimate the cross-pose from a small number of demonstrations of a given task, generalizing to novel objects within the training categories.
To complete the manipulation task, we use the estimated cross-pose as the target of a motion planning algorithm, which will move the objects into the desired configuration (e.g. placing the mug onto the rack, placing the lasagna into the oven, etc).

 
\begin{wrapfigure}[25]{r}{0.4\linewidth}
    \centering
    \includegraphics[width=\textwidth, trim={0 0 0 0},clip]{figures/corl-teaser-fig-grid.pdf}
    \vspace{-10pt}
    \caption{We study relative placement tasks, in which one object needs to be placed in a position relative to another object. Here are two of the tasks that we demonstrate our method on: \textbf{Top:} \textit{PartNet-Mobility Placement Task} requires one object (e.g. a block) to be placed relative to another object (e.g. a drawer) by a semantic goal position (e.g. inside); \textbf{Bottom:} \textit{Mug Hanging Task} requires placing the mug's handle on the mug rack.}
    \label{teaser}
    \vspace{-10pt}
\end{wrapfigure}


In this paper, we present TAX-Pose (TAsk-specific Cross-Pose), a deep 3D vision-based method that learns to predict a task-specific pose relationship between a pair of objects from a set of demonstrations. 
%We use this predicted pose relationship to plan a trajectory that moves the objects into the desired relative pose. 
Our cross-pose estimation system is provably translation equivariant and can generalize from a small number of real-world demonstrations (in some cases as few as 10) to new objects in unseen poses. 

The contributions of this paper include:
\begin{enumerate}[nosep,leftmargin=*]
    % \item A novel goal pose prediction model based on a demonstration from another instance.
    \item A precise definition of ``cross-pose," which defines a task-specific pose relationship between two objects.
    \item A novel method that estimates soft-correspondences between two objects, from which the cross-pose between the objects can be estimated (see Figure~\ref{fig:teaser_pipeline}); this method is provably translation equivariant and can learn from a small number of real-world demonstrations.
    \item  A  robot system to manipulate objects into the desired cross-pose to achieve a given manipulation task. 
\end{enumerate}

We present simulated and real-world experiments to test the performance of our system in achieving a variety of relative placement manipulation tasks. %, learning from a small number of demonstrations. %We show that our model can generalized to novel objects, accurately hanging unseen mugs and interacting with a large variety of placement objects.
We demonstrate our method on 
%We show the generalizabilty of our model though 
a semantic placement task, in which the robot must place an object in, on, or around a novel object (Figure \ref{teaser}, top). We also demonstrate our method on precise placement tasks, such as hanging a mug on a rack (Figure \ref{teaser}, bottom) or placing a bottle or bowl on a shelf; in both cases our method generalizes to new object configurations and new objects within the training categories.

 

==> taxpose/sec-2-rw.tex <==


\textbf{Object Pose Estimation}:
Pose estimation is the task of detecting and inferring the 6DoF pose of an object, which includes its position and orientation, with respect to some previously defined object reference frame~\cite{lowe1999object,rothganger20063d,xiang2017posecnn,he2020pvn3d,he2021ffb6d,turpin2021gift}. Recent work~\cite{manuelli2019kpam,qin2020keto, vecerik2021s3k,manuelli2021keypoints, pan2023tax} proposed to use 3D semantic keypoints as an alternative form of object representation. While keypoint-based methods can generalize within an object class, they require a significant amount of hand annotated data or access to a simulated version of the task to learn to estimate the keypoint locations. In contrast, our method is able to learn from just 10 real-world demonstrations. Another approach is to use dense embeddings, such as Dense Object Nets (DON)~\cite{florence2018dense, zhang2016health} and Neural Descriptor Fields (NDF)~\cite{simeonov2021neural, zhang2021robots},
which achieve generalization across classes by predicting dense embeddings in the observation and matching them to embeddings of the demonstration objects. However, DON~\cite{florence2018dense, zhang2023flowbot++} and NDF~\cite{simeonov2021neural, sim2019personalization} assume that the target object is moved relative to a static reference object  in a ``known canonical configuration" (e.g. the pose of the mug rack in NDF~\cite{simeonov2021neural} is assumed to be known and fixed). In contrast, our method reasons about the %``cross-pose" which describes a task-specific
geometric relationship between a pair of objects and hence does not need to assume a static environment. Thus, for example, our method is able to perform the mug hanging task while varying the pose of the mug rack (see our \href{https://sites.google.com/view/tax-pose/home}{project website}), whereas the baselines (DON~\cite{florence2018dense}, NDF~\cite{simeonov2021neural}) cannot. Further, we show that our method significantly outperforms both the DON~\cite{florence2018dense} and NDF~\cite{simeonov2021neural} baselines, especially when given a very small number of demonstrations. 

\textbf{Point Cloud Registration}: Our method for estimating the cross-pose between two objects builds upon previous work in point cloud registration. The typical objective in point cloud registration is to find the optimal rigid alignment between two point clouds, to minimize the sum of squared distances between two sets of points. Traditionally, Iterative Closest Point (ICP)~\cite{besl1992method, zhang2020dex} and its variants~\cite{bouaziz2013sparse, rusinkiewicz2001efficient, segal2009generalized,agamennoni2016point, hinzmann2016collaborative, hahnel2002probabilistic} have been used to compute the optimal rigid alignment between two point clouds.
Deep Closest Point (DCP)~\cite{wang2019deep} avoids local minima common for ICP by seeking to approximate correspondence in a high-dimensional learned feature space.  Our method builds upon the architecture of DCP for cross-pose estimation; however, in contrast to point cloud registration, in which the objective is to minimize the sum of squared distances between two sets of points on the same object in two different poses, our objective is to estimate a task-specific pose relationship between two different objects.
%From a technical standpoint, our work is the first to introduce the notion of cross-pose, which we define as a function of cross-object correspondences in Section~\ref{sec:Problem Statement}. 
Extending the framework from DCP, we learn a residual to the soft correspondences, allowing for points to match outside the convex hull of each object. This component is necessary when computing soft correspondences between objects of drastically different morphologies (such as a mug and a mug rack).  

==> taxpose/sec-3-ps.tex <==
% Given two objects $\mathcal{A}$ and $\mathcal{B}$, where object $\mathcal{A}$ is immobile and $\mathcal{B}$ is free to move, we suppose there are multiple possible relations between $\mathcal{A}$ and $\mathcal{B}$ defined by the relative pose ${}_\mathcal{A}T^\mathcal{B}$ between them, where ${}_\mathcal{A}T^\mathcal{B}\in SO(3)$. We conjecture that different relative poses are able to define different semantic positions between the two objects such as ``inside'' and ``on top of''. This is fairly common in household scenarios, where the semantic goals of the tasks are defined by a relative geometric relation. Modeling such relational distribution is difficult due to its multi-modality. To alleviate this issue, we also define a set of ``demo'' objects, where each set of demo objects contains two objects   $\mathcal{A}_d$ and  $\mathcal{B}_d$ where $\mathcal{B}_d$ is placed relative to $\mathcal{A}_d$ with pose ${}_{\mathcal{A}_d}T_g^{\mathcal{B}_d}$, where ${}_{\mathcal{A}_d}T_g^{\mathcal{B}_d}$ is able to convey the goal $g$ defined by the relative pose between $\mathcal{A}_d$ and  $\mathcal{B}_d$. This set of demo objects are used to condition the decision-making process to match the semantic meaning conveyed by goal $g$.




% DON'T DELETE: THIS IS BEN'S UGLY BUT PRECISE DEFINITION.

% G_{AB} := \text{Frame} \to (\text{Pose} \to \text{Pose}) \\ 
% \text{The goal relationship function, which maps a frame to a function of a pose} \\ \\

% G_{AB}(F) := \text{Pose} \to \text{Pose} \\ 
% \text{A function which maps the pose of B expressed in F to the} \\ 
% \text{concrete pose of A expressed in F which achieves the goal relationship} \\

% \\ \\

% X_{G_{AB}} := \text{Frame} \to ((\text{Pose} \times \text{Pose}) \to \text{Transform}) \\ 
% \text{The cross-pose function function, which takes a Frame in and outputs a function which calculates cross-pose} \\

% X_{G_{AB}}(F) := X_{G_{AB}(F)} := (\text{Pose} \times \text{Pose}) \to \text{Transform} \\
% \text{The cross-pose function, which takes as input two poses:} \\
% \text{The current pose of A expressed in F, and the current pose of B expressed in F} \\
% \text{The function returns the cross-pose, which transforms A into A', such that:} \\
% T_{A'F} = G_{AB}(F)(T_{BF})  \\ \\

% \text{In other words:} \\
% T_{A'A} = X_{G_{AB}(F)}(T_{AF}, T_{BF}) \\
% T_{A'F} = G_{AB}(F)(T_{BF}) = X_{G_{AB}(F)}(T_{AF}, T_{BF}) \cdot T_{AF} \\ \\



% P_{AF} := \text{Current A points in some frame F}

% P_{A'F} := \text{Desired A points in some frame F}

% P_{BF} := \text{B points in some frame F} \\ \\

% \text{This formulation allows us to swap out A poses expressed in F for points expressed in F}: \\

% P_{A'F} = X_{G_{AB}(F)}(T_{AF}, T_{BF}) \cdot P_{AF}



% \text{The learning problem then becomes}:
% f_{\theta}(P_{AF}, P_{BF}) = X_{G_{AB}(F)}(T_{AF}, T_{BF})


\section{Problem Statement}
\label{sec:Problem Statement}

\begin{wrapfigure}[16]{R}{0.4\textwidth}
    \begin{center}
    \vspace{-10pt}
    \includegraphics[width=\textwidth, trim={0 0 0 0}, clip]{figures/corl-rel_placement.pdf}
    \vspace{-20pt}
    \end{center}
    \caption{If we transform both the action object (mug) and the anchor object (rack) by the same transform, then the relative pose between these objects is unchanged (the mug is still ``on" the rack) so the mug is still in the goal configuration. 
    % \dave{It seems that we don't refer to this figure anywhere in the text.  We should figure out where to reference it.  One thought - this figure really shows the definition of a relative placement task, so it should probably be moved to the section where we define relative placement tasks (and referred to there in the text) - although in that case maybe the equations beneath the figures should be removed?}
    }
    \label{fig:rel_placement}
\end{wrapfigure}

\textbf{Relative placement tasks:}
In this paper, we are specifically interested in ``relative placement tasks."   Given two objects, $\mathcal{A}$ and $\mathcal{B}$, a ``relative placement task" is the task of placing object $\mathcal{A}$ at a pose relative to object $\mathcal{B}$. For example, consider the task of placing a lasagna in an oven, placing a mug on a rack, or placing a robot gripper on the rim of a mug.  All of these tasks involve placing one object (which we call the ``action'' object $\mathcal{A}$) at a semantically meaningful location relative to another object (which we call the ``anchor'' object $\mathcal{B}$)\footnote{Note that the definition of action and anchor is symmetric; either object can be treated as the action object and the other as the anchor. }. 
%Intuitively, a relative placement task is a task such that  only the relationship between objects $\MA$ and $\MB$ is important for task success.  



% \ben{I kind of feel we should be more explicit about reference frames here. What we want to say is: `this is the pose of A expressed in the coordinate frame of F'. One way to write this would be $T_{AF}$, which is what Murray-Lee-Sastry do. Therefore you could say, ``Suppose that $\mathbf{T}_{\MA F}^*$ and $\mathbf{T}_{\MB F}^*$ are poses for objects $\MA$ and $\MB$ respectively in some arbitrary reference frame $F$ (the body frame of $B$, for instance, might be a common reference frame to choose as $F$)... Importantly, the body frames of A and B are also arbitrary: we can choose to place the body frame anywhere relative to the mass of the object (centroid is commonly used); what is not arbitrary is the relationship between the objects when described in a single frame (i.e. F).}
%chuer{I kind of echo Ben's views, below is my }
Specifically, suppose that $\mathbf{T}_{\MA}^*$ and $\mathbf{T}_{\MB}^*$ 
are $SE(3)$ poses for objects $\MA$ and $\MB$ respectively (in a shared world reference frame\footnote{All $SE(3)$ transformations in this work are defined in a fixed, arbitrary world frame.}) for which a desired task is considered complete (lasagna is in the oven; mug is on the rack, etc). Then for a relative placement task, if objects $\MA$ and $\MB$ are in poses $\mathbf{T} \cdot \mathbf{T}_{\MA}^*$ and $\mathbf{T} \cdot \mathbf{T}_{\MB}^*$ (respectively) for any transform $\mathbf{T}$, then the task will also be considered to be complete, as seen in Figure~\ref{fig:rel_placement}.  
% In other words, if $\mathbf{T}_{\MB}^*$ represents the pose of the oven and $\mathbf{T}_{\MA}^*$ represents the pose of the lasagna in that oven (at task completion); then if we transform the both the lasagna and oven poses by $\mathbf{T}$, then the lasagna will still be located inside the oven.
In other words, if $\mathbf{T}_{\MB}^*$ represents the pose of the rack and $\mathbf{T}_{\MA}^*$ represents the pose of the mug on the rack (at task completion); then if we transform the both the mug and rack poses by $\mathbf{T}$, then the mug will still be located on the rack.
Formally, this property can be defined with the following Boolean function,
\begin{equation}
    \text{RelPlace}(\mathbf{T_\MA}, \mathbf{T_\MB}) = \textbf{\textsc{Success}}  \text{ iff}~\exists \mathbf{T} \in SE(3) \text{ s.t. } \mathbf{T_{\MA}} = \mathbf{T} \cdot \mathbf{T_{\MA}^{*}} \text{ and } \mathbf{T_{\MB}} = \mathbf{T} \cdot \mathbf{T_{\MB}^{*}}.
\label{eq:relplace_def_simple}
\end{equation}
% \dave{We have formally defined relative placement tasks in Appendix X.} \dave{Or we can add the definition here, it's pretty short}\chuer{addded}
%OLD VERSION:
%We first define the notion of a ``relative placement task." 
%Relative placement tasks can either admit a single unambiguous solution (i.e. placing an asymmetric object in a specific pose, such as inserting an asymmetric peg into a hole), or a set of solutions (e.g. when there are object symmetries, or when the goal is semantically defined, such as ``place the object somewhere on top of the table'').  
For many real semantic placement tasks, there are actually sets of valid solutions which solve each task (i.e., there are many potential locations to place an object on a table to achieve a semantic ``object-on-table'' relationship). However, for this work, we consider precise placement tasks under the simplifying assumption that, for a given pose of object $\mathcal{B}$, there is a single, unambiguous pose of object $\MA$ needed to achieve the task.
 
% In this work, we make the simplifying assumption that, for a given pair of objects $\mathcal{A}$ and $\mathcal{B}$, there is a single, unambiguous relative pose needed to achieve a given task.

%Thus, we treat $\mathcal{A}$ as an ``action'' object, and $\mathcal{B}$ as an ``anchor'' object \footnote{Note that the definition of action and anchor is symmetric.}. 

% \dave{Brian - please edit this}
% \rebuttal{In this work, we consider only placement tasks where there is a single, unambiguous solution for how an object should be placed. In other words, for a given pair objects, we assume there is }

\textbf{Definition of Cross-Pose:}  Given the above definition of a relative placement task, our goal will be to determine how to move object $\MA$ so that it will be in the ``goal pose," which, as described above, is defined relative to the pose of object $\MB$. To achieve this, one option is to estimate the poses of objects $\MA$ and $\MB$ separately and then compute the transformation needed to move object $\MA$ into the goal pose. However, the pose estimate of each object will have errors, and these errors will accumulate when the poses are combined  into the single relative pose needed to reach the goal configuration. 
%Further, training a pose estimator requires pose annotations, whereas we only require a small number of demonstrations.
%combining them to estimate the transformation needed to achieve the goal pose.

Instead of estimating the pose of each object independently, we aim to learn a function  $f(\mathbf{P}_\mathcal{A}, \mathbf{P}_\mathcal{B})$, which takes as input the point clouds $\mathbf{P}_\mathcal{A}$ and $\mathbf{P}_\mathcal{B}$ for both objects $\MA$ and $\MB$ %(respectively)
,
% where $\mathbf{P}_k \in \mathbb{R}^{3\times N_k}$, and $N_k$ denotes the number of 3D points in the point cloud of object $k$. 
 where $\mathbf{P}_{\MA} \in \mathbb{R}^{3\times N_{\MA}}$ and $\mathbf{P}_{\MB} \in \mathbb{R}^{3\times N_{\MB}}$ are 3D point clouds of sizes $N_{\MA}$ and $N_{\MB}$, respectively.
 This function outputs an SE(3) rigid transformation,
% \begin{equation}
$f(\mathbf{P}_\mathcal{A}, \mathbf{P}_\mathcal{B}) = \mathbf{T}_{\mathcal{A}\mathcal{B}}$,
% \end{equation}
where we refer to $\mathbf{T}_{\mathcal{A}\mathcal{B}}$ as the ``cross-pose" between object $\mathcal{A}$ and object $\mathcal{B}$. For notational convenience, we occasional write $f$ as a function of the poses $\mathbf{T}_{\MA}$, $\mathbf{T}_{\MB}$ of point clouds $\PA$ and $\PB$ respectively (with respect to a global reference frame) such that $f(\mathbf{T}_{\MA}$, $\mathbf{T}_{\MB}) := f(\PA, \PB)$. This notational change is to make the transformation math more intuitive; in practice, this function only ever receives point clouds as input.


We will define the cross-pose $\mathbf{T}_{\mathcal{A}\mathcal{B}}$ (below) such that, if we transform  object $\mathcal{A}$ by $\mathbf{T}_{\mathcal{A}\mathcal{B}}$, then object $\MA$ will be in the goal pose relative to object $\MB$ for the relative placement task.  For example,  suppose that $\mathbf{T}_{\MA}^*$ and $\mathbf{T}_{\MB}^*$
are poses for objects $\MA$ and $\MB$, respectively, for which a desired relative placement task is considered complete. 
In this configuration, the cross-pose of these objects would be  $f(\mathbf{T}_{\MA}^*, \mathbf{T}_{\MB}^*) = \mathbf{I}$ where $\mathbf{I}$ is the identity, as object $\MA$ does not need to be moved to complete the task.
% ; in other words, we do not need to move object $\MA$ at all to achieve the task. 
Further, based on the definition of a relative placement task given above, if both objects are transformed by the same transform $\mathbf{T}$, then the objects will still be in the desired relative pose, 
    \begin{equation}
 f(\mathbf{T} \cdot \mathbf{T}_{\MA}^*, \mathbf{T} \cdot \mathbf{T}_{\MB}^*) = f( \mathbf{T}_{\MA}^*, \mathbf{T}_{\MB}^*) = \mathbf{I}
    \label{eq:transform_both}
    \end{equation}
    for any transform $\mathbf{T} \in SE(3)$. Now, let us assume that objects $\MA$ and $\MB$ are not in the goal configuration and have pose $\mathbf{T}_{\MA} = \mathbf{T}_\alpha \cdot \mathbf{T}_{\MA}^*$ and $\mathbf{T}_{\MB} = \mathbf{T}_\beta \cdot \mathbf{T}_{\MB}^*$, respectively, for arbitrary transforms $\mathbf{T}_\alpha$ and $\mathbf{T}_\beta \in SE(3)$. We then define the ``cross-pose" of objects $\MA$ and $\MB$ as:
%and a current ``cross-pose" of
% \begin{equation}
% f(\mathbf{T}_\alpha \mathbf{T}_{\MA}^*,  \mathbf{T}_\beta \mathbf{T}_{\MB}^*):= %\mathbf{T}_\alpha \mathbf{T}_{\MA \MB}^* \mathbf{T}_\beta^{-1} = 
% %\mathbf{T}_\alpha \cdot \mathbf{T}_\beta^{-1}.
% \mathbf{T}_\beta \cdot \mathbf{T}_\alpha^{-1}.
% \label{eq:usability-cross-pose}
% \end{equation}
\begin{equation}
f(\mathbf{T}_{\MA}, \mathbf{T}_{\MB}) = f(\mathbf{T}_\alpha\cdot  \mathbf{T}_{\MA}^*,  \mathbf{T}_\beta \cdot \mathbf{T}_{\MB}^*) = \mathbf{T}_{\MA\MB}:= \mathbf{T}_\beta \cdot \mathbf{T}_\alpha^{-1}.
\label{eq:usability-cross-pose}
\end{equation}
Note that this definition is equivalent to Equation~\ref{eq:transform_both} for the special case of $\mathbf{T}_\alpha = \mathbf{T}_\beta$. 
This definition of cross-pose allows us to move object $\MA$ into the goal configuration, relative to object $\MB$: \begin{equation}
\mathbf{T}_{\mathcal{A}\mathcal{B}} \cdot \mathbf{T}_{\MA} = (\mathbf{T}_\beta \cdot \mathbf{T}_\alpha^{-1}) \cdot (\mathbf{T}_\alpha \cdot \mathbf{T}_{\MA}^*) = \mathbf{T}_\beta \cdot \mathbf{T}_{\MA}^*, 
\end{equation}
satisfying the relative placement condition defined in Equation~\ref{eq:relplace_def_simple} with $\mathbf{T} = \mathbf{T}_\beta$. Alternatively, we could  have instead transformed  object $\MB$ by the inverse of the cross-pose to achieve the task.


==> taxpose/sec-4-methods-2.tex <==
% This is just a clean scratch page to fiddle with the text of methods.

% \newcommand{\MA}[0]{{\mathcal{A}}}
% \newcommand{\MB}[0]{{\mathcal{B}}}

% \newcommand{\PA}[0]{\mathbf{P}_{\MA}}
% \newcommand{\PB}[0]{\mathbf{P}_{\MB}}
% \newcommand{\NA}[0]{N_{\MA}}
% \newcommand{\NB}[0]{N_{\MB}}
% \newcommand{\TAB}[0]{\mathbf{T}_{\MA \MB}}

% \newcommand{\AtoB}[0]{\MA \to \MB}
% \newcommand{\BtoA}[0]{\MB \to \MA}

% \newcommand{\VA}[0]{\mathbf{\tilde{V}}_{\MA}}
% \newcommand{\VB}[0]{\mathbf{\tilde{V}}_{\MB}}
% \newcommand{\VA}[0]{\mathbf{\tilde{V}}_{\mathcal{A}\to \mathcal{B}}}
% \newcommand{\VB}[0]{\mathbf{\tilde{V}}_{\mathcal{B}\to \mathcal{A}}}

\textbf{Overview:}
We frame the task of cross-pose estimation as a soft correspondence-prediction task between a pair of point clouds, followed by an analytical least-squares optimization to find the optimal \textit{cross-pose} for the predicted correspondences. As described in Appendix \ref{appendix:proof}, this correspondence-based approach allows our method to be translation-equivariant: translating either object ($\mathcal{A}$ or $\mathcal{B}$) will lead to a translated cross-pose prediction.
%We will show that this framing allows our cross-pose estimator to be provably translation-equivariant, 
This allows our method to automatically adapt to novel positions of both the anchor and action objects, unlike previous work which assumes a static anchor~\cite{simeonov2021neural}. %Under this framing, we present TAX-Pose, a model that estimates the task-specific cross-pose from a learned soft correspondence prediction. 
Our method for task-specific cross-pose estimation, known as TAX-Pose, consists of the following steps, as shown in Figure~\ref{fig:gc-ipm}:

\begin{figure*}[b]
    \centering
    % \includegraphics[width=\textwidth, trim={20 50 10 240}, clip]{figures/system_figures/system_figure_ab.png}
    \includegraphics[width=\textwidth, clip]{figures/system_figures/system_figure_ab_new.png}
    \vspace{-20pt}
    \caption{TAX-Pose Training Overview: Given a specific task, our method takes as  input two point clouds and outputs the cross-pose between them needed to achieve the task. TAX-Pose first learns point clouds features using two DGCNN~\cite{phan2018dgcnn} networks and two Transformers~\cite{vaswani2017attention}. Then the learned features are each input to a point residual network to predict per-point soft correspondences and weights across the two objects. The desired cross-pose can be inferred analytically from these correspondences using singular value decomposition.}
    \label{fig:gc-ipm}
\end{figure*}

\begin{enumerate}[leftmargin=*]
    \item \textbf{Soft Correspondence Prediction}: For a pair of objects $\mathcal{A, B}$, a neural network learns to predict a per-point embedding to establish a (soft) correspondence between $\mathcal{A}$ and $\mathcal{B}$, which are called ``virtual soft correspondences." The corresponding points are constrained to be within the convex hulls of $\mathcal{B}$ and $\mathcal{A}$ respectively.
    \item \textbf{Adjustment via Correspondence Residuals}: 
For most estimation tasks,  some points in object $\mathcal{A}$ may not be within the convex hull of object $\mathcal{B}$;
%in direct contact with any point in object $\mathcal{B}$; 
for instance, when a mug is placed on a mug rack, most points on the mug will be outside of the convex hull of the mug rack.
%not be in direct contact with any point on the rack.  
To accommodate these cases, we apply a pointwise residual vector to displace each of the predicted soft correspondences. These ``corrected virtual correspondences" allow points in $\mathcal{A}$ to correspond to locations in free space near $\mathcal{B}$.

    \item \textbf{Find the Optimal Transform}: Because the cross-pose is defined as a rigid transformation of object $\MA$, we use a differentiable weighted SVD to find the transformation that minimizes the weighted least squares difference to the corrected virtual correspondences.
\end{enumerate}


 

Because each step above is differentiable, the whole model can be optimized end-to-end, despite having an interpretable internal structure which we describe below.
%our method can learn arbitrary correspondences that solve arbitrary cross-pose estimation tasks. 
Our method is heavily inspired by Deep Closest Point (DCP) \cite{wang2019deep}. The key difference between our pose alignment model and DCP is that we predict the cross-pose between two \emph{different} objects for a given task instead of registering two point clouds of an identical object. Additionally, TAX-Pose can predict relationships where these clouds may not have any points of contact or overlap. 

We now describe our cross-pose estimation algorithm in detail. To recap the problem statement, given objects $\MA$ and $\MB$ with point cloud observations $\PA$ $\in \mathbb{R}^{3\times N_{\mathcal{A}}}$, $\PB$ $\in \mathbb{R}^{3\times N_{\mathcal{B}}}$  respectively, our objective is to estimate 
the task-specific cross-pose $\TAB = f(\PA, \PB) \in SE(3)$. Note that the cross-pose between object $\MA$ and $\MB$ is defined with respect to a given task (e.g. putting a lasagna in the oven, putting a mug on the rack, etc).




\subsection{Cross-Pose Estimation via Soft Correspondence Prediction}
\label{sec:soft_corr}
\textbf{Soft Correspondence Prediction}: The first step of the method is to compute two sets of correspondences between $\MA$ and $\MB$, one which maps from points in $\MA$ to $\MB$, and one which maps from points in $\MB$ to $\MA$. These need not be a bijection, and can be asymmetric. 
As we want each step to be differentiable, we 
follow DCP's conventions and estimate a \textit{soft correspondence}. This assigns a \textit{virtual soft corresponding point} $\mathbf{v}_{i}^{\mathcal{A}}\in \mathbf{V}_{\mathcal{A}}$ to every point $\mathbf{p}_{i}^{\MA} \in \PA$ by computing a convex combination of points in $\PB$, and vice versa. Formally:\\
\begin{subequations}
\begin{minipage}{.5\textwidth}
    \begin{equation} 
        \mathbf{v}_{i}^{\mathcal{A}} = \PB \mathbf{w}_{i}^{\AtoB}  \quad \text{s.t.} \quad \sum_{j=1}^{N_{\MB}} w_{ij}^{\AtoB} = 1
    \end{equation}
\end{minipage}%
\hfill
\begin{minipage}{.5\textwidth}
    \begin{equation} 
        \mathbf{v}_{i}^{\mathcal{B}} = \PA \mathbf{w}_{i}^{\BtoA}  \quad \text{s.t.} \quad \sum_{j=1}^{N_{\MA}} w_{ij}^{\BtoA} = 1    
        % \label{soft_correspondence}
        \end{equation}
\end{minipage}
\label{soft_correspondence}
\end{subequations}
with normalized weight vectors $\mathbf{w}_{i}^{\AtoB} \in \mathbf{W}_{\AtoB}$ and $\mathbf{w}_{i}^{\BtoA} \in \mathbf{W}_{\BtoA}$. Importantly, these virtual corresponding points are not constrained to the surfaces of $\MA$ or $\MB$; instead, they are constrained to the convex hulls of $\PB$ and $\PA$, respectively. 

To compute the weights %$\mathbf{W}_{\AtoB}$, $\mathbf{W}_{\BtoA}$ 
$\mathbf{w}_{i}^{\AtoB}$, $\mathbf{w}_{i}^{\BtoA}$  in Equations~\ref{soft_correspondence}a and~\ref{soft_correspondence}b, we first encode each point cloud $\PA$ and $\PB$ into a latent space using a neural network encoder, DGCNN~\cite{phan2018dgcnn}. This encoder head is comprised of two distinct encoders $g_{\MA}$ and $g_{\MB}$, each of which receives point cloud $\PA$ and $\PB$, respectively, zero-centers them, and outputs a dense, point-wise embedding for each object (see Figure~\ref{fig:gc-ipm}):
%\begin{equation}
     $\boldsymbol{\Psi}_\mathcal{A} = g_{\mathcal{A}}(\bar{\mathbf{P}}_{\mathcal{A}}) \in \mathbb{R}^{N_{\mathcal{A}}\times d},\;\;
     \boldsymbol{\Psi}_\mathcal{B} = g_{\mathcal{B}}(\bar{\mathbf{P}}_{\mathcal{B}})\in \mathbb{R}^{N_{\mathcal{B}}\times d}$
     %$\Phi_\mathcal{A} = g_{\mathcal{A}}(\mathbf{P}_\mathcal{A}),\;\;
     %\Phi_\mathcal{B} = g_{\mathcal{B}}(\mathbf{P}_\mathcal{B})$
% \end{equation}
where $\boldsymbol{\psi}_i^{\mathcal{K}} \in \boldsymbol{\Psi}_\mathcal{K}$ is the $d$-dimensional embedding of the $i$-th point in object $\mathcal{K}$, and $\bar{\mathbf{P}}_{\mathcal{K}}$
%:=\mathbf{P}_{\mathcal{K}} - \frac{1}{N_\mathcal{K}} \sum_{i=1}^{N_k} \mathbf{P}_\mathcal{K} \in \mathbb{R}^{3 \times N_{\mathcal{K}}}$ 
is the zero-centered point cloud for object $\mathcal{K}$. 
Because we want the cross-correspondence to incorporate information about both point clouds, we then employ a cross-object attention module between the two dense feature sets 
to obtain \textit{cross-object point embeddings},
$\boldsymbol{\Phi}_{\mathcal{A}} \in \mathbb{R}^{N_\mathcal{A}\times d}$ and $\boldsymbol{\Phi}_{\mathcal{B}} \in \mathbb{R}^{N_\mathcal{B}\times d}$, defined as: 
\begin{equation}
    \boldsymbol{\Phi}_{\mathcal{A}} = \boldsymbol{\Psi}_{\mathcal{A}} + g_{\mathcal{T}_{\mathcal{A}}}(\boldsymbol{\Psi}_{\mathcal{A}}, \boldsymbol{\Psi}_{\mathcal{B}}) , \;\; 
    \boldsymbol{\Phi}_{\mathcal{B}} = \boldsymbol{\Psi}_{\mathcal{B}} + g_{\mathcal{T}_{\mathcal{B}}}(\boldsymbol{\Psi}_{\mathcal{B}}, \boldsymbol{\Psi}_{\mathcal{A}})
\end{equation}
where $g_{\mathcal{T}_{\mathcal{A}}}$,
$g_{\mathcal{T}_{\mathcal{B}}}$ are Transformers~\cite{vaswani2017attention}. 


Finally, %to map our estimated features to a set of normalized weights 
recall that our goal was to compute a set of normalized weight vectors $\mathbf{W}_{\AtoB}$, $\mathbf{W}_{\BtoA}$. To compute the virtual corresponding point $\mathbf{v}_i^{\MA}$ assigned to any point $\mathbf{p}_i^{\MA}\in \mathbf{P}^{\MA}$, we can extract the desired normalized weight vector $\mathbf{w}_{i}^{\AtoB}$ from intermediate attention features of the cross-object attention module as:
\begin{equation}
    \mathbf{w}_{i}^{\AtoB} = \text{softmax}\left(\frac{\mathbf{K_{\MB}}\mathbf{q}_{i}^{\MA}}{\sqrt{d}}\right), \;\;
     \mathbf{w}_{i}^{\BtoA} = \text{softmax}\left(\frac{\mathbf{K_{\MA}}\mathbf{q}_{i}^{\MB}}{\sqrt{d}}\right) \;\;
\end{equation}
where $\mathbf{q}_i^{\mathcal{K}} \in \mathbf{Q_{\mathcal{K}}}$, and $\mathbf{Q_{\mathcal{K}}}, \mathbf{K_{\mathcal{K}}} \in \mathbb{R}^{\mathbf{N}_{\mathcal{K}}\times d}$ are the query and key values (respectively) for object $\mathcal{K}$ associated with cross-object attention Transformer module $g_{\mathcal{T}_{\mathcal{K}}}$ (see Appendix \ref{appendix:cross-object-weight}~for details). These weights are then used to compute the virtual soft correspondences $\mathbf{V}_{\mathcal{A}}$, $\mathbf{V}_{\mathcal{B}}$ using Equation\cameraready{~\ref{soft_correspondence}.}


\textbf{Adjustment via Correspondence Residuals:} 
As previously stated, the virtual soft correspondences  $\mathbf{V}_{\mathcal{A}}, \mathbf{V}_{\mathcal{B}}$ given by Equations~\ref{soft_correspondence}a and~\ref{soft_correspondence}b are constrained to be within the convex hull of each object. However, many relative placement tasks cannot be solved perfectly with this constraint.
% correspondences which are constrained to the convex hull are insufficient to express 
For instance, we might want a point on the handle of a teapot to correspond to some point above a stovetop (which lies outside the convex hull of the points on the stovetop). To allow for such off-object correspondences, we further learn a \textit{residual vector}, $\boldsymbol{\delta}_{i}^{\mathcal{A}} \in \boldsymbol{\Delta}_{\mathcal{A}}$ for each 
%point-wise embedding $\boldsymbol{\phi}_i$ 
point $i$
that corrects each virtual corresponding point $\mathbf{v}_{i}^{\mathcal{A}}$. This allows us to displace each virtual corresponding point to any arbitrary location that might be suitable for the task. To compute these residual vectors, we use a point-wise neural network $g_{\mathcal{R}_\MA}$, $g_{\mathcal{R}_\MB}$ to map each point's embedding into a 3D residual vector:
\begin{equation*}
    \boldsymbol{\delta}_i^{\mathcal{A}} = g_{\mathcal{R}_\MA} \left(\boldsymbol{\phi}_i^{\MA}\right) \in \mathbb{R}^3,\;\; 
     \boldsymbol{\delta}_i^{\mathcal{B}} = g_{\mathcal{R}_\MB} \left(\boldsymbol{\phi}_i^{\MB}\right) \in \mathbb{R}^3
\end{equation*}
Applying these residual offsets to the virtual points, we get a set of \textit{corrected virtual correspondences}, $\tilde{\mathbf{v}}_i^{\mathcal{A}} \in \VA$ and $\tilde{\mathbf{v}}_i^{\mathcal{B}} \in \VB$,  defined as
%\cameraready{$\VA = \begin{bmatrix} \tilde{v}_1^{\AtoB} \dots \tilde{v}_{\NA}^{\AtoB} \end{bmatrix}^\top$ and $\VB =  \begin{bmatrix} \tilde{v}_1^{\BtoA} \dots \tilde{v}_{\NB}^{\BtoA} \end{bmatrix}^\top$, where $\tilde{v}_i^{\AtoB}$ and $\tilde{v}_i^{\BtoA}$ are defined as,}
\begin{equation}
    \tilde{\mathbf{v}}_i^{\mathcal{A}} = \mathbf{v}_i^{\mathcal{A}} + \boldsymbol{\delta}_i^{\mathcal{A}},\;\; 
    \tilde{\mathbf{v}}_i^{\mathcal{B}} = \mathbf{v}_i^{\mathcal{B}} + \boldsymbol{\delta}_i^{\mathcal{B}} 
\end{equation}
These corrected virtual correspondences $\tilde{\mathbf{v}}_i^{\mathcal{A}}$ define the estimated goal location relative to object $\MB$ for each point $\mathbf{p}_i \in \PA$ of object $\MA$, and likewise for each point in object $\MB$ (see visualization in Appendix~\ref{appendix:illustration}).



\textbf{Least-Squares Cross-Pose Optimization with Weighted SVD:}
Given the sets of dense correspondences, $\left(\PA, \VA\right)$ and $\left(\PB, \VB\right)$, we would like to compute a single rigid transformation for object $\MA$.  To do so, we solve for the transformation $\TAB$ (the cross-pose) that minimizes the weighted distance between each point and its corrected virtual correspondence.
% For point cloud $\PA$, we have now computed the set of corrected virtual correspondences $\VA$, which is the network's estimate of where each point in $\PA$ would need to move to in order to be in the goal position relative to object $B$ (see Figure S1 in Appendix E.1.).  Likewise, for point cloud $\PB$, we have computed the set of corrected virtual correspondences $\VB$. However, because $\PA$ is assumed to be a rigid object, it cannot independently move each point to the corresponding location in $\VA$.  Instead, we solve for a rigid transformation $\TAB$ (the cross-pose) that minimizes the weighted distance between points and their correspondences. 
Formally, this leads to the following weighted least squares optimization:
\begin{equation}
    \mathcal{J}(\TAB) = \sum_{i=1}^{\NA} \alpha_i^{\MA} || \TAB~\mathbf{p}_{i}^{\MA} - \tilde{\mathbf{v}}_i^{\MA} ||_2^2 + \sum_{i=1}^{\NB} \alpha_i^{\MB} || \TAB^{-1}~\mathbf{p}_{i}^{\MB} - \tilde{\mathbf{v}}_i^{\MB} ||_2^2
    \label{eq:weighted_least_squares}
\end{equation}
where the weights $\alpha_i^{\MA} \in \boldsymbol{\alpha}_{\MA}$, $\alpha_i^{\MB} \in \boldsymbol{\alpha}_{\MB}$ signify the importance of each correspondence and are predicted by a point-wise MLP as shown in Figure~\ref{fig:gc-ipm}. These weights are 
learned end-to-end as parameters of our network; they are visualized in Appendix \ref{appendix:importance_weights},
%the third stage of Figure~\ref{fig:gc-ipm},
which shows that the network has learned to assign more weight to the parts of the object that are most important for the task, such as the region around the mug handle (on the mug) and the region around the peg (on the rack). Equation~\ref{eq:weighted_least_squares} is the well-known weighted Procrustes problem, for which there exists an analytical solution. %As shown in Figure~\ref{fig:gc-ipm}, 
To maintain the differentiablity of the system, we use a weighted differentiable SVD operation~\cite{papadopoulo2000estimating} to compute the cross-pose $\TAB$ that minimizes this objective
(see Appendix \ref{appendix:weighted-svd}~for details). This allows us to train the system end-to-end as described below. 

\subsection{TAX-Pose Training Pipeline}

To train our model, we use a segmented set of demonstration point clouds of a pair of objects in the goal configuration. For each demonstration point cloud, we generate multiple training examples by  transforming each object's point cloud, $\PA$ and $\PB$ by random SE(3) transformations $\mathbf{T}_\alpha$ and $\mathbf{T}_\beta$, respectively. The predicted cross-pose, $\TAB$, is then compared with the ground truth cross-pose, $\TAB^{GT} :=\mathbf{T}_{\beta}\mathbf{T}_{\alpha}^{-1}$, using an average distance loss~\cite{hinterstoisser2012model} with dense regularization (see more details on our training losses in Appendix \ref{appendix:training-supervision}).



==> taxpose/sec-5-exps.tex <==
To evaluate TAX-Pose, we conduct a wide range of simulated and real-world experiments on two classes of relative placement tasks: NDF~\cite{simeonov2021neural} Tasks and PartNet-Mobility  Placement Tasks. All tasks involve placing an ``action" object at a specific location relative to an anchor object, in which the relative pose is specified by a set of demonstrations. Our method then generalizes to perform this task on novel objects in unseen configurations.
%The Object Placement objective is to place an action object on a flat surface on or near an anchor object. The Mug Hanging task objective is to grasp and then hang unseen mugs on a rack. 
We refer the reader to our \href{https://sites.google.com/view/tax-pose/home}{project website} for additional results and videos.

\subsection{NDF Tasks}
\label{sec:NDF Tasks}
\looseness=-1
We evaluate our method on all three NDF~\cite{simeonov2021neural, devgon2020orienting} tasks (\textit{mug} hanging, \textit{bottle} placement, and \textit{bowl} placement); see Appendix \ref{appendix:results-ndf-bowlbottle} for results on \textit{bottle} and \textit{bowl} placement. Results on \textit{mug} hanging are described in more detail below.

\textbf{Simulation Experiments:}
For our simulation experiments, we perform the task of hanging a mug on a rack as two sequential cross-pose estimation  steps: grasping the mug (estimating the cross-pose between the gripper and the mug) and hanging the mug on the rack (estimating the cross-pose between the mug and the rack). 
In Pybullet \cite{coumans2020, avigal20206, avigal2021avplug}, we simulate a Franka Panda above a table with 4 depth cameras placed on the corners of the table. The model is trained on 10 simulated demonstrations of mug hanging. We evaluate task execution success on unseen mug instances in randomly generated initial configurations.
% To successfully execute the manipulation task of hanging a mug on a rack by the mug's handle requires the successful inference of two sequential task-specific cross-poses: 1) predict a successful grasp pose; 2) predict the hanging pose of mug relative to the rack. 
% In the first stage, it requires our model to reason about the cross-pose between the gripper and the mug, while the second stage requires prediction of the cross-pose between the mug and the rack. We utilize Pybullet \cite{coumans2016pybullet} and simulate a Franka Panda arm situated above a table with 4 depth cameras placed at each table corner. For training, the model is provided with 10 demonstrations in simulation, each on a different mug instances. At test time, we measure the task execution success on unseen mug instances, with randomly generated initial poses. 
% To evaluate robustness to different initial poses, we evaluate on two sets of initial poses: 1) \textit{Upright Pose}: where the mug is initialized to have an upright orientation, and placed randomly on the surface of the table; 2) \textit{Arbitrary Pose}: where the mug is initialized to have arbitrary orientation and position, irrespective of table surface is.
We measure task success rates of 1) \textit{Grasping}, where success is achieved when the object is grasped stably; 2) \textit{Placing}, where success is achieved when the mug is placed stably on the rack; 3)  \textit{Overall}, when the predicted transforms enable both grasp and place success in sequence. We compare our method to Neural Descriptor Field (NDF)~\cite{simeonov2021neural} and Dense Object Nets (DON)~\cite{florence2018dense}. Details of these methods can be found in prior work~\cite{simeonov2021neural, zhang2021robots}. 
%Dense Object Nets (DON)~\cite{florence2018dense} and Neural Descriptor Fields (NDF)~\cite{simeonov2021neural}.

% \underline{Dense Object Nets (DON)}~\cite{florence2018dense}: Using manually labeled semantic keypoints on the demonstration clouds, DON is used to compute sparse correspondences with the test objects. These correspondences are converted to a pose using SVD. A full description can be found in~\cite{simeonov2021neural}.

% \underline{Neural Descriptor Field (NDF)}~\cite{simeonov2021neural}: Using the learned descriptor field for the mug, the positions of a constellation of task specific quarry points are optimized to best match the demonstration using gradient descent.
\textbf{Simulation Results:}
We evaluate our method in simulation in 100 trials consisting of unseen \textit{mug} instances in random initial and goal configurations for both \textbf{Upright} and \textbf{Arbitrary} poses. 
%We compare the performance of our method against DON~\cite{florence2018dense} and NDF~\cite{simeonov2021neural}. 
As shown in Table~1, our method significantly outperforms the baselines 
%See Table~2 for results 
for simulated mug hanging. We report  additional results for simulated \textit{bottle} and \textit{bowl} placement tasks in Table \ref{tab:bottle_bowl} in Appendix \ref{appendix:results-ndf-bowlbottle}.

\looseness=-1
\textbf{Ablation Analysis: } \textit{Effects of Number of Demonstrations.} To study how the number of demonstrations observed affects our method's performance, we train our model on \{10, 5, 1\} demonstrations of upright pose mug hanging. Results are found in Table~2. Our method outperforms the baselines for all number of demonstrations; TAX-Pose can perform well even with as few as 5 demonstrations. 

\textit{Cross-Pose Estimation Design Choices.} We analyze the effects of design choices made in our Cross-Pose estimation algorithm for the upright pose mug hanging task. Specifically, we analyze the effects of 1) computing residual correspondence; 2) the use of \textit{weighted} SVD over non-weighted in computing cross-pose; 3) using a transformer as the cross-object attention, as opposed to simpler model such as a 3-layer MLP.  Table~3 shows that each major component of our system is important for task success. See more ablation experiments in Appendix \ref{appendix:results-ndf-ablations}.

\input{tables/ablation_fewshot}
% \input{tables/ablation_fewshot}

% \textbf{Ablation Analysis.} 
% \textit{Number of Demonstrations.} To study the effects of number of demonstrations used on the performance of our method, we report quantitative performance of our method alongside baseline methods trained on different numbers of demonstrations (10, 5, 1) for upright pose mug hanging task as seen in Table 4. Our method outperforms the baselines for all number of demonstrations; TAX-Pose can perform well even with just 5 demonstrations.
%~\ref{tab:mug_on_rack_few_shot}
%We find that our method is able to retain high success rates relatively better than the baselines with fewer demonstrations used.\newline
% \input{tables/mug_on_rack_few_shot}

% \textit{Cross-Pose Estimation Design Choices.} We analyze the effects of the different design choices made in our Cross-Pose estimation algorithm for the upright pose mug hanging task. Specifically, we analyze the effects of 1) computing residual correspondence; 2) the use of \textit{weighted} Procrustes over the non-weighted in computing cross-pose; 3) using a transformer as the cross-object attention as in Figure \ref{fig:gc-ipm} method, as opposed to simpler model such as a 3-layer MLP. We report results in Table 5. %~\ref{tab:mug_rack_ablation}.
% \input{tables/mug_rack_ablation}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/newrwsummary_aligned.pdf}
     \vspace{-20pt}
    \caption{Real-world experiments summary. \textbf{Left: } In object placement task, we train using simulated demonstrations and test on real-world objects. \textbf{Right: }Mug Hanging real-world experiments. We train from just 10 demonstrations from 10 training mugs in the real world and test on 10 unseen test mugs. 
    %In real-world experiments, the robot observes the starting segmented point clouds of the mug and the rack, and infers the cross-pose between them using TAX-Pose. The robot then grasps the mug using a primitive and once contact is made, the robot executes a motion plan that executes the predicted relative transform. \dave{I'm not sure this whole explanation is necessary in the caption}
    }
    \label{fig:mughangingrw}
    
\end{figure}

\label{sec:mug_hanging}
\textbf{Real-World Experiments: } 
We explore the 
%extension of the 
hanging component of the mug on a rack task in a real world environment, which requires 
estimating the cross-pose between the mug and the rack.
%Our real-world mug-hanging experiments show our method's ability to make precise pose predictions on real-world data. 
We train TAX-Pose using real demonstrations of 10 different mugs hung on a rack (1 demonstration each, for a total of only 10 real-world demonstrations for training). A motion primitive is used to grasp each mug, after which the robot plans a trajectory to apply the predicted cross-pose to the grasped mug. 
%, and restrict the learning task to predicting the relationship between the mug and rack (ignoring the gripper-mug relationship). 
We evaluate the model on the 10 training mugs in novel poses, as well as on  10 unseen mugs (see Figure~\ref{fig:mughangingrw}). For each of the 20 mugs, we conduct 5 trials, varying the mug's and rack's starting poses in each trial. Success is recorded if a peg penetrates the mug handle at the end of the trial. Our method achieves a success rate of 62\% on training mugs in novel poses and 54\% on unseen mugs. A visualization of the results can be seen in Figure~\ref{fig:mughangingrw} (right) and on the \href{https://sites.google.com/view/tax-pose/home}{project website}. Note that our method is able to perform the mug hanging task while varying the pose of the mug rack (see our \href{https://sites.google.com/view/tax-pose/home}{project website}), whereas the baselines (NDF~\cite{simeonov2021neural}, DON~\cite{florence2018dense}) cannot because they assume a fixed, known rack position (see NDF~\cite{simeonov2021neural} for baseline details).


% While our method is able to accurately predict relative transforms required to achieve a given task, it does require an accurate segmentation of the objects of importance. Additionally, while our method is tested with some occlusions, it performs better with a mostly complete cloud of the object being manipulated. This means that multiple views of that object must be captured. This can be done with multiple cameras, or by lifting the object and capturing multiple views. 
% Additionally, in our experiments, we have found that the predicted rotation is not always accurate enough to hang the virtual mugs given the small number of demonstrations. In the case that more accurate estimates are required,
% Additionally, as our method is a function of correspondences, multimodal target configurations can cause potential problems. Such multimodalites can occur when interacting with symmetric objects or when the task has multiple valid configurations, such as objects with multiple valid placement surfaces, or racks with multiple usable hangers. These problems could be alleviated using a consensus-based method for mapping from multimodal soft correspondences to a single transform.  We leave this for future work.

% results suggest that the accuracy of our predicted rotations can ..\ben{Mention goal sets}



\subsection{PartNet-Mobility  Placement Tasks}
\textbf{Task Description}: We also define a PartNet-Mobility Placement task as placing a given action object relative to an anchor object based on a semantic goal position. We select a set of household furniture objects from the PartNet-Mobility dataset~\cite{Xiang2020-oz} as the anchor objects, and a set of small rigid objects released with the Ravens simulation environment \cite{zeng2020transporter, yao2023apla, jin2024multi, shen2024diffclip} as the action objects. For each anchor object, we define a set of semantic goal positions (i.e. `top', `left', `right', `in'), where action objects should be placed relative to each anchor. Each semantic goal position defines a unique task in our cross-pose prediction framework. Given a synthetic point cloud observation of both objects, the task is to predict a cross-pose that places the object at the specific semantic goal. 
We evaluate both a \emph{goal-conditioned} variant (\textbf{TAX-Pose GC}), which is trained across all goals, and a \emph{task-specific} variant (\textbf{TAX-Pose}) of our model, which trains a separate model per goal type (see Appendix~\ref{appendix:results-pm-gc} for details). In both cases we train only 1 model across all action and anchor objects.
All models are trained entirely on simulated data and transfer directly to real-world with no finetuning. Further task details can be found in the Appendix \ref{appendix:taskdetails-pm}.
% MOVE TO APPENDIX
% \textbf{Simulation Setup. }The selected subset of the dataset contains 9 categories of objects. We split the objects into 58 seen and 16 unseen instances. During training, for a specific task of each of the seen objects, we generate an action-anchor objects pair by randomly sampling transformations from $SE(3)$ as cross-poses. The action object is chosen from the Ravens simulator's rigid body objects dataset \cite{Zeng2020-tk}. 
% The ground-truth cross-pose is then defined by this specific task. For each observation action-anchor objects pair, we sample 100 times using the aforementioned procedure for the training dataset. During testing, for each tested observation anchor object we randomly construct 20 test scenes using the same steps. 
% During training, for each of the 58 seen objects, we generate a demonstration action-anchor objects pair by choosing a random goal from the defined semantic goals. The demonstration action object is randomly chosen from the Ravens simulator's rigid objects \cite{Zeng2020-tk}, and the demonstration anchor object is randomly chosen from the subset of PartNet-Mobility dataset. We then place the demonstration action object relative to the demonstration anchor object based on the ground-truth pose of the goal. Subsequently, we also randomly define an observation action-anchor pair, where the action object is chosen from the same dataset but placed randomly in the scene and the anchor object is a random object of the same category as that of the demonstration object. Note that in the simulated experiments, we only consider translation, so the rotation of each object is always identity. For each observation anchor object, we sample 200 times using the aforementioned procedure for the training dataset. During testing, for each tested observation anchor object we randomly construct 20 test scenes using the same steps. 
% \harry{TODO: TASK here IS OVERLOADED... WE HAVE TWO TASKS (PM DATASET and MUG), but for PM DATASET TASK< WE ALSO DEFINE 4 TASKS for ANCHOR-ACTION PAIR...}


%We report the following metrics on a held-out set of anchor objects in simulation:
% \begin{itemize}
%     \item \textit{Translational Error}: The L2 distance between the inferred cross-pose translation ($\mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{pred}$) and the ground-truth pose translation ($\mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{GT}$).
%     \item \textit{Rotational Error}: The minimal angular offset \cite{Wat} between the predicted cross-pose rotation ($\mathbf{R}_{\mathcal{A}\mathcal{B}}^\mathrm{pred}$) and the ground-truth cross-pose rotation ($\mathbf{R}_{\mathcal{A}\mathcal{B}}^\mathrm{GT}$).
% \end{itemize}

% \begin{tabular}{@{}p{.48\textwidth}p{.48\textwidth}@{}} % Remove margins left and right.
%      \textit{Translational Error}: The L2 distance between the inferred cross-pose translation ($\mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{pred}$) and the ground-truth pose translation ($\mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{GT}$). & 
%      \textit{Rotational Error}: The geodesic $SO(3)$ distance between the predicted cross-pose rotation ($\mathbf{R}_{\mathcal{A}\mathcal{B}}^\mathrm{pred}$) and the ground-truth rotation ($\mathbf{R}_{\mathcal{A}\mathcal{B}}^\mathrm{GT}$).
%      \\
%      \parbox{0.5\textwidth}{\begin{equation*} 
%         \mathcal{E}_\mathbf{t} = ||\mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{pred} - \mathbf{t}_{\mathcal{A}\mathcal{B}}^\mathrm{GT}||_2
%     \end{equation*}} 
%      & 
%      \parbox{0.5\textwidth}{\begin{equation*} 
%         \mathcal{E}_\mathbf{R} = \frac{1}{2} \arccos{\left(\frac{\mathrm{tr}(\mathbf{R}_{\mathcal{A}\mathcal{B}}^{\mathrm{pred}\top} \mathbf{R}_{\mathcal{A}\mathcal{B}}^\mathrm{GT})-1}{2}\right)}
%     \end{equation*}}
% \end{tabular}

% Specifically, we test both goal-inference and downstream execution independently.
% \textit{Goal-Inference}. We first compute the goal-inference normalized Chamfer distance between the ground-truth goal point cloud and the inferred goal point cloud. The metric is computed as:
% \begin{equation}
%     \mathcal{E}_\mathrm{goal} = \frac{\mathrm{Chamf}\left(\mathbf{P}_\mathcal{A}''\oplus \mathbf{P}_\mathcal{B}, [\mathbf{T}^{\mathrm{GT}}_{\mathcal{A}\mathcal{B}}]\mathbf{P}_\mathcal{A}\oplus \mathbf{P}_\mathcal{B}\right)}{\mathrm{Chamf}\left(\mathbf{P}_\mathcal{A}\oplus \mathbf{P}_\mathcal{B}, [\mathbf{T}^{\mathrm{GT}}_{\mathcal{A}\mathcal{B}}]\mathbf{P}_\mathcal{A}\oplus \mathbf{P}_\mathcal{B}\right)}
% \end{equation}
% We also define a binary success rate for goal inference, which is computed by thresholding the final resulting normalized distance at $\epsilon:\mathrm{Success} = \mathbbm{1}(\mathcal{E}_\mathrm{goal} \leq 0.1)$. We set $\epsilon=0.1$, meaning that we define a success as the normalized distance between the inferred goal point cloud and ground-truth goal point cloud less than 0.1. 
% Results of goal inference in simulated experiments are shown in Table \ref{tab:gi-chamfer-dist} and \ref{tab:gi-sr}\footnote{Categories from left to right: microwave, chair, dishwasher, oven, fridge, table, washing machine, safe, and drawer.}.
% \textit{Execution}. We then compute a separate normalized distance for the downstream execution. We define the execution normalized L2 distance as the distance between the ground truth action object goal pose and the executed goal pose:
% \begin{equation}
%     \mathcal{E}_\mathrm{exec} = \frac{||\mathbf{T}^{\mathrm{GT}}_{\mathcal{A}\mathcal{B}} - \hat{\mathbf{T}}_{\mathcal{A}\mathcal{B}}||_2}{||\mathbf{T}^{\mathrm{GT}}_{\mathcal{A}\mathcal{B}} - \mathbf{T}^{0}_{\mathcal{A}\mathcal{B}}||_2}
% \end{equation}
% We also define a binary success rate for goal inference, which is computed by thresholding the final resulting normalized distance at $\epsilon:\mathrm{Success} = \mathbbm{1}(\mathcal{E}_\mathrm{exec} \leq 0.1)$, \textit{conditioned on a collision-free path}. We set $\epsilon=0.1$ as well.
% \textbf{Baselines}: We compare our method to the a variety of imitation-learning-based methods trained from a motion planner expert in simulation. Specifically, we train an \underline{E2E Behavioral Cloning} agent from the offline expert data, an \underline{E2E DAgger} \cite{ross2011reduction} agent from the offline expert data and test-time corrections \dave{``Test-time corrections" is not a good way to describe this}, a \underline{Trajectory Flow} \cite{EisnerZhang2022FLOW} agent using the same DAgger dataset but represents the action with a dense flow field \dave{Seems unclear}, and a \underline{Goal Flow} agent that outputs dense flow directly pointing to the goal pose \dave{It seems that we don't have enough room to clearly describe these baselines.  Please just say: ``

\textbf{Baselines}: We compare our method to a variety of end-to-end imitation-learning-based methods trained from a motion planner expert in simulation (see Appendix \ref{appendix:taskdetails-pm-baselines} for details). Note that in the PartNet-Mobility Placement experiments, the pose of the anchor object poses are randomly varied. As such, we omit a comparison to methods that assume a static anchor, such as the Neural Descriptor Field (NDF)~\cite{simeonov2021neural} and Dense Object Nets (DON)~\cite{florence2018dense} baselines used in the mug hanging task (Section~\ref{sec:NDF Tasks}), as both methods
%DON~\cite{florence2018dense} and NDF~\cite{simeonov2021neural} 
%compare directly to the objects demonstration poses and 
assume that the anchor objects are in a fixed, known position. 
% Comparison to these baseline methods is reserved for Section~\ref{sec:mug_hanging}.

% \underline{E2E Behavioral Cloning}: Generate motion-planned trajectories using OMPL that take the action object from start to goal. These serve as ``expert'' trajectories for Behavioral Cloning (BC), where we train a neural network to output a policy that, at each time step, outputs an incremental 6-DOF transformation that imitates the expert trajectory. %The ``prediction'' is the final achieved state of the action object.

% \underline{E2E DAgger}: Using the same BC dataset as above, we train a policy using DAgger~\cite{ross2011reduction}.
    
% \underline{Trajectory Flow}: Using the same BC dataset with DAgger, we train a policy to predict a dense per-point 3D flow vector at each time step instead of a single incremental 6-DOF transformation. Given this dense per-point flow, we can extract a rigid transformation using SVD yielding the next pose.
    
% \underline{Goal Flow}: Instead of training a multi-step policy to reach the goal, train a network to output a single dense prediction which assigns a per-point 3D flow vector that points from each action object point directly to its corresponding goal location. We extract a rigid transformation from these flow vectors using SVD, yielding the goal pose.



% BEN COMMENTED THIS OUT JUST TO TRY SOMETHING.
% \input{tables/gi-chamfer-dist-merged}
% \input{tables/gi-sr-rate-merged}
% \input{tables/exec-l2-dist-merged}
% \input{tables/exec-sr-rate-merged}

% \input{tables/single_goal}


% \begin{figure*}[h]

%     % \centering
    
%     \caption{Real-world experiments illustration. \textbf{Left: }workspace setup for physical experiments. The sensory signal comes from an Azure Kinect depth camera, and the agent is a Franka Panda robot. \textbf{Right: }Octomap representation of the anchor object in ROS's RViz interface for motion planning via MoveIt!.}
%     \label{workspace}
% \end{figure*}

% \begin{figure}
% \begin{floatrow}
% \ffigbox{%
%   \includegraphics[width=0.5\textwidth]{figures/realworld-setup.pdf}%
% %   \vspace{-15pt}
% }{%
%   \caption{Real-world experiments illustration. \textbf{Left: }workspace setup for physical experiments. The sensory signal comes from an Azure Kinect depth camera, and the agent is a Franka Panda robot. \textbf{Right: }Octomap representation of the anchor object in ROS's RViz interface for motion planning via MoveIt!.}\label{workspace}}
% \capbtabbox{%
% \resizebox{0.5\textwidth}{!}{
%   \begin{tabular}{|r|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
% \tiny{Goal Flow} & 0.18 & 0.38 & 0.37 \\ \hline
% \tiny{\textbf{TAX-Pose}} & 0.95 & 0.95 & 0.85 \\ \hline
% \end{tabular}
% }}{%
%   \caption{A table}%
% }
% \end{floatrow}
% \end{figure}

% \begin{table}[ht]
\begin{wraptable}[12]{r}{0.26\linewidth}
\vspace{-12pt}
% \begin{minipage}{\textwidth}
% % \begin{minipage}[b]{0.4\linewidth}
% %     \centering
% %     \includegraphics[width=\textwidth]{figures/realworld-setup.pdf}
% %     \captionof{figure}{Real-world experiments illustration. \textbf{Left: }work-space setup for physical experiments. \textbf{Center: }Octomap visualization of the perceived anchor object.} 
% %     \label{fig:image}
% % \end{minipage}%
% % % \qquad
% % \hfill
% \begin{minipage}[b]{0.5\linewidth}
%     \renewcommand{\arraystretch}{1.2}
    \resizebox{0.9\textwidth}{!}{
%     \setlength\tabcolsep{.2em}
%     % \begin{tabular}{|lr|cc|}
%     % \hline
%     %  \rule{0pt}{0.5em}
%     %  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ Average}}\\ 
%     %  & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
%     % \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.26 & 0.73 \\
%     % \multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 37.96 & 0.69  \\ \hline
%     % \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.95 & 0.67 \\
%     % \multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 26.64 & 0.17  \\
%     % % \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
%     % \hline
%     % \multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.64} & \textbf{0.16} \\ 
%     % % \multicolumn{1}{|l|}{} & \textbf{TAX-Pose GC} & 7.74 & 0.17\\
%     % \hline
%     % \end{tabular}
%     % Please add the following required packages to your document preamble:
%     % \usepackage{multirow}
%     \begin{tabular}{|l|ll|}
%     \hline
%     \multirow{2}{*}{} & \multicolumn{2}{c|}{Average} \\
%     & \multicolumn{1}{c}{$\mathcal{E}_\mathbf{R}$} & \multicolumn{1}{c|}{$\mathcal{E}_\mathbf{t}$} \\ \hline
%     E2E BC & 42.26 & 0.73 \\ \hline
%     E2E DAgger & 37.96 & 0.69 \\ \hline
%     Traj. Flow \cite{EisnerZhang2022FLOW} & 35.95 & 0.67 \\ \hline
%     Goal Flow & 26.64 & 0.17 \\ \hline
%     \textbf{TAX-Pose} & \textbf{6.64} & \textbf{0.16} \\ \hline
%     \end{tabular}
%     }
% \label{tab:gi-Rt}
% \vspace{1em}
% \end{minipage}
% % \hfill
% \begin{minipage}[b]{0.45\linewidth}
% % \small
% \centering
%     \renewcommand{\arraystretch}{1.2}
%     % \resizebox{\textwidth}{!}{
%     % \begin{tabular}{ |r|c|c|c|}
%     %     \hline
%     %     \rule{0pt}{2.5em} & \clipart{drawer} & \clipart{fridge} & \clipart{oven}\\ \hline
%     %     Goal Flow & 0.18 & 0.38 & 0.37 \\ \hline
%     %     \textbf{TAX-Pose} & \textbf{0.95} &\textbf{0.95} & \textbf{0.85} \\ \hline
%     % \end{tabular}
%     % }
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{ |r|c|}
%         \hline
%         \rule{0pt}{0.5em} & Average SR\\ \hline
%         Goal Flow & 0.31 \\ \hline
%         \textbf{TAX-Pose} & \textbf{0.92} \\ \hline
%     \end{tabular}
%     }
% % \captionof{table}{Real-world goal placement success rate }
% \label{table:real-world}
% \vspace{2em}
% \end{minipage}
% \end{minipage}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lll}
\hline
\multicolumn{1}{|l|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Average} \\
\multicolumn{1}{|l|}{} & \multicolumn{1}{c}{$\mathcal{E}_\mathbf{R}$} & \multicolumn{1}{c|}{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{E2E BC} & 42.26 & \multicolumn{1}{c|}{0.73} \\ \hline
\multicolumn{1}{|l|}{E2E DAgger} & 37.96 & \multicolumn{1}{l|}{0.69} \\ \hline
\multicolumn{1}{|l|}{Traj. Flow} & 35.95 & \multicolumn{1}{l|}{0.67} \\ \hline
\multicolumn{1}{|l|}{Goal Flow} & 26.64 & \multicolumn{1}{l|}{0.17} \\ \hline
\multicolumn{1}{|l|}{TAX-Pose} & 6.64 & \multicolumn{1}{l|}{\textbf{0.16}} \\ \hline
% \multicolumn{1}{|l|}{TAX-Pose GC} & 7.74 & \multicolumn{1}{l|}{0.17} \\ \hline
\multicolumn{1}{|l|}{\textbf{TAX-Pose GC}} & \textbf{4.94} & \multicolumn{1}{l|}{\textbf{0.16}} \\ \hline

 &  &  \\ \hline
\multicolumn{1}{|l|}{} & \multicolumn{2}{c|}{Average SR} \\ \hline
\multicolumn{1}{|l|}{Goal Flow} & \multicolumn{2}{c|}{0.31} \\ \hline
\multicolumn{1}{|l|}{\textbf{TAX-Pose}} & \multicolumn{2}{c|}{\textbf{0.92}} \\ \hline
\end{tabular}

}
% \vspace{10pt}
\caption{\textbf{Top}: Simulation Rotational ($^\circ$) and Translational ($\mathrm{m}$) Errors ($\downarrow$). \textbf{Bottom}: Real-world goal placement success rate ($\uparrow$).}
\label{tab:2tables}
\end{wraptable}
% \qquad
% \begin{varwidth}[b]{0.33\linewidth}
    
% \end{varwidth}%
% \end{table}
% \vspace{-1em}
% \begin{figure}[tbp]
%   \centering
%   \begin{minipage}[t]{0.65\linewidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/realworld-setup.pdf}
%   \end{minipage}
%   \hspace{0.02\linewidth}
%     % \qquad
%     % \resizebox{0.2\textwidth}{!}{
%   \begin{minipage}[t]{0.3\linewidth}
%     \centering
%       \begin{tabular}{|r|c|c|c|}
%         \hline
%         \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
%         \tiny{Goal Flow} & \tiny{0.18} & \tiny{0.38} & \tiny{0.37} \\ \hline
%         \tiny{\textbf{TAX-Pose}} & \tiny{0.95} & \tiny{0.95} & \tiny{0.85} \\ \hline
%     \end{tabular}
%     % }
%   \end{minipage}
%   \caption{Real-world experiments illustration. \textbf{Left: }workspace setup for physical experiments. The sensory signal comes from an Azure Kinect depth camera, and the agent is a Franka Panda robot. \textbf{Right: }Octomap representation of the anchor object in ROS's RViz interface for motion planning via MoveIt!.}
%   \label{workspace}
% \end{figure}
% Results of full execution in simulated experiments are shown in Table \ref{tab:exec-l2-dist} and \ref{tab:exec-sr}.
% For both goal-inference and full execution evaluations, we test the baselines methods with action object's initial poses that are inside the training distribution (``In'' columns of the tables) and outside the training distribution (``Out'' columns of the tables).

% \textbf{Real-World Experiments}: We design a set of of real world experiments to evaluate the performance of our cross-pose prediction model on real objects. We choose several real-world furniture objects similar to those found in the simulated training categories, annotate semantic goal locations for each, and choose several analogous action objects (bowl, block) to place at the goals. For each semantic goal, the task is to predict the appropriate cross-pose directly from point clouds recorded by a depth camera and have a Franka Emika Panda robot place the action object at the cross-pose. We compare TAX-Pose and the Goal Flow baseline for pose estimation. As ground-truth cross-pose is hard to define in the real-world, we qualitatively define a ``goal region'' for each anchor object. Success is defined as the inferred pose of the action object landing inside the goal region of the anchor object. Details can be found in Appendix H.3. \dave{This section seems to be heavily overlapping with ``Task Description."  Can we cut it?  Is there anything in this section that we need to keep?}

\textbf{Results}:  We report rotation ($\mathcal{E}_\mathbf{R}$) and translation ($\mathcal{E}_\mathbf{t}$) error between our predicted transform and the ground truth as geodesic rotational distance~\cite{huynh2009metrics, hartley2013rotation, elmquist2022art, teng2024gmkf} and $L2$ distance, respectively. In both our simulated experiments (Table~\ref{tab:2tables} Top) and our real-world experiments (Table~\ref{tab:2tables} Bottom), we find that TAX-Pose outperforms the baseline end-to-end imitation learning methods, with the \emph{goal-conditioned} variant, TAX-Pose GC, performing the best. 
%In simulated experiments, while direct regression via goal-flow outperforms TAX-Pose in some rare cases of translation prediction, TAX-Pose performs substantially better than all other baselines in rotation prediction. 
In real-world experiments, our method generalizes to novel distributions of starting poses better than the Goal Flow baseline, placing action objects into the goal regions with a 92\% success rate.
See Figure~\ref{fig:mughangingrw} (left) and the \href{https://sites.google.com/view/tax-pose/home}{website} for results; 
see Appendix \ref{appendix:results-pm} for more detailed tables and Appendix \ref{appendix:taskdetails-pm-baselines} for baseline details.  


%(see Figure~\ref{fig:mughangingrw} (left) for a result illustration, see Appendix \ref{appendix:results-pm} for more detailed results and Appendix \ref{appendix:taskdetails-pm-baselines} for baseline details.).  
% due to the provably translation-equivariant property of TAX-Pose, i

% , where we manipulate a variety of different household objects to achieve cross-pose prediction and execution on similar  tasks using a Franka Emika Panda robot in our workspace, as shown in Fig. \ref{workspace}. We select 3 tasks for our physical experiments: placing the action object inside, on top of, and to the left of the anchor object. We compare TAX-Pose with the Goal Flow baseline. Our experiment protocol is thus: for each given task, each action-anchor objects pair in the real-world dataset, we conduct 10 trials of each method. For each trial, the action and anchor objects are placed in the scene at random positions such that the surfaces are visible and the robot can reach every position in the range of motion of each goal. The policy is then executed in an open-loop fashion: first we collect the point cloud data and do inference, and then we grasp the action object using pre-defined grasp primitives and then actuate it to the inferred goal pose. In real-world experiments, we first clean up the point cloud and filter out ground planes and noise following the same procedure in \cite{EisnerZhang2022FLOW}. Then we obtain a clean mask for the action object using position thresholding and motion planning is done by avoiding an Octomap  reconstruction based on the anchor object point cloud. 

% \subsection{Mug Hanging}

 

==> taxpose/sec-6-conclusion.tex <==
In this paper, we show that dense soft correspondence can be used to learn task specific object relationships that generalize to novel object instances. Correspondence residuals allow our method to estimate correspondences to virtual points, outside of the objects convex hull, drastically increasing the number of tasks this method can complete. We further show that this ``cross-pose" can be learned for a task, using a small number of demonstrations. Finally, we show that our method far outperforms the baselines on two challenging tasks in both real and simulated experiments. While our method is able to predict relative pose relationships with high precision, it has several limitations:
\begin{itemize}[leftmargin=*]
    \item \textbf{Requires segmentation}: Our method requires an accurate segmentation of two objects in order to predict their relative goal pose.
    \item \textbf{Performance degrades under occlusion}: Our method performs best when complete point clouds are provided, captured via multiple cameras or by repeatedly reorienting the objects.
    \item \textbf{Poorly defined for multimodal relationships}: Because our method extracts a single global estimate of relative pose from a fixed set of correspondences, performance on objects with multiple valid goals is not well-defined. Our method might be augmented with a consensus-based or sampling-based approach to capture the multimodality of the solution space in these cases. We leave this for future work.
\end{itemize}
\section*{Acknowledgements}
{\footnotesize
This material is based upon work supported by the National Science Foundation under Grant No. IIS-1849154. This work was also supported by LG Electronics. We are grateful to Daniel Seita and Jenny Wang for their helpful feedback and discussion on the paper.
}

==> taxpose/tables/ablation-in-main.tex <==
% \begin{table}[ht]
% \begin{varwidth}[b]{0.1\linewidth}
%     \centering
%       \renewcommand{\arraystretch}{1}
%     %  \resizebox{6\linewidth}{!}{
%     \begin{tabular}{c|c c c}
%     % \hline
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%  % }
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \qquad
% \begin{varwidth}[b]{}
%     \centering
%       
%      
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%      
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%



% \end{table}


% \begin{table}[htb]
    \begin{minipage}[t]{.3\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        }
        \captionof{table}{ \# Demos vs. Overall Success}

    \end{minipage}%
    \hfill
    \begin{minipage}[t]{.4\textwidth}
        % \small
        \centering
        \label{tab:mug_rack_ablation}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c| c c c}
    \hline
  \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
        % \textit{Loss}&&&\\
          No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
          No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
           No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
            Scaled Combination: 
            %of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ (
            $ 1.1\mathcal{L}_\mathrm{cons} + \mathcal{L}_\mathrm{corr}$ &  0.10 & 0.01 & 0.01 \\
         \hline 
          No Adjustment via Correspondence Residuals  & 0.97 &0.96 & 0.93\\
         \hline 
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
        \hline 
         No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
         No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         \hline 
         3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
        \hline
        Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
        \hline
        \hline
        \textbf{TAX-Pose (Ours)}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
    \hline
    \end{tabular}
    }
        \captionof{table}{Mug Hanging Ablations Results}

    \end{minipage}%
% \end{table}


==> taxpose/tables/ablation_attention_weight.tex <==
 

\begin{table}[H]
 
    \centering
\renewcommand{\arraystretch}{1}
 
    \begin{tabular}{c|c c c}
    
        \hline
        \textbf{Attention Weight Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
        \hline
        Point Embedding Dot-Product (Eqn.~\ref{eq:point embedding dot-product}) & 0.83 & 0.92 & 0.92\\
        \textbf{TAX-Pose (Ours) (Eqn.~\ref{eq:TAXPose-weight-computation})} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
        \hline
    
    \end{tabular}
   
    
    \caption{Test success rate ($\uparrow$) over 100 trials for mug hanging upright task, ablated on attention weight computation methods.}
    \label{tab:ablation_weight}
\end{table}



 

==> taxpose/tables/ablation_fewshot.tex <==
% \begin{table}[ht]
% \begin{varwidth}[b]{0.1\linewidth}
%     \centering
%       \renewcommand{\arraystretch}{1}
%     %  \resizebox{6\linewidth}{!}{
%     \begin{tabular}{c|c c c}
%     % \hline
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%  % }
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \qquad
% \begin{varwidth}[b]{}
%     \centering
%       
%      
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%      
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%



% \end{table}


% \begin{table}[htb]
    
    
    \noindent \begin{minipage}[t]{.45\textwidth}
    % \vspace{0.5em}
    
    \label{tab:mug_on_rack_exp}
    % \small
        \centering
        \resizebox{\textwidth}{!}{
%         \begin{tabular}{c| c c c}
%     \hline
%   \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%         % \textit{Loss}&&&\\
%           No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
%           No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
%           No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
%             Scaled Combination: 
%             %of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ (
%             $ 1.1\mathcal{L}_\mathrm{cons} + \mathcal{L}_\mathrm{corr}$ &  0.10 & 0.01 & 0.01 \\
%          \hline 
%           No Adjustment via Correspondence Residuals  & 0.97 &0.96 & 0.93\\
%          \hline 
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%         \hline 
%          No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
%          No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
%          \hline 
%          3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
%         \hline
%         Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
%         \hline
%         \hline
%         \textbf{TAX-Pose (Ours)}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
%     \hline
%     \end{tabular}

%\begin{table}[h]
\begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    \label{tab:mug_on_rack_exp2}
    %\end{table}
    }
    \captionof{table}{Mug on rack simulation success rate ($\uparrow$)}
    
    \end{minipage}%
    \hfill
    \noindent \begin{minipage}[t]{.24\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        }
        \vspace{-2pt}
        
        \captionof{table}{ \# Demos vs. Overall success rate ($\uparrow$)}
    \end{minipage}%
    \hfill
    \begin{minipage}[t]{.28\textwidth}
        % \small
        \centering
        \label{tab:mug_rack_ablation}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
            \hline
            No Res.  & 0.97 &0.96 & 0.93\\
            Unw. SVD &  0.92 & 0.94 & 0.88 \\
            %  3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
            No Attn. &  0.90 & 0.82 & 0.76 \\
            \textbf{TAX-Pose} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
            \hline
        \end{tabular}
        }
        \captionof{table}{Mug hanging ablations success rate ($\uparrow$)}

    \end{minipage}%
% \end{table}


==> taxpose/tables/bottle_bowl_results.tex <==
\begin{table}[H]
    % \small
    \centering
     
\resizebox{0.7\textwidth}{!}{
    \begin{tabular}{c|c|c c c| c c c}
    \hline
   \textbf{Object} & \textbf{Algorithm}& \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
    & & \multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
    \multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Mug}}} & DON \cite{florence2018dense} & 0.91 & 0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
        & NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
        & \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75 & \textbf{0.84}& \textbf{0.63}\\
    \hline
    
    \multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Bowl}}} & DON \cite{florence2018dense} & 0.50 & 0.35 & 0.11 & 0.08 & 0.20 & 0 \\
        & NDF \cite{simeonov2021neural} & 0.91 & \textbf{1} & 0.91  & \textbf{0.79} & \textbf{0.97} & 0.78\\
        & \textbf{TAX-Pose (Ours)} & \textbf{0.99}& 0.92 & \textbf{0.92} &  0.74 & 0.85& \textbf{0.85}\\
    \hline
    
    \multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Bottle}}} & DON \cite{florence2018dense} & 0.79 & 0.24 & 0.24 & 0.05 & 0.02 & 0.01 \\
        & NDF \cite{simeonov2021neural} & \textbf{0.87} & \textbf{1} & \textbf{0.87} & \textbf{0.78} & \textbf{0.99} & \textbf{0.77} \\
        & \textbf{TAX-Pose (Ours)} & 0.55 & 0.99 & 0.55 &  0.61 & 0.55 & 0.52\\
         
    \hline
 
    \end{tabular}
    }
    \caption{Unseen Object Instance Manipulation Task Success Rates ($\uparrow$) in Simulation on \textit{Mug}, \textit{Bowl} and \textit{Bottle} for Upright and Arbitrary Initial Pose. Each result is the success rate over 100 trials.} 
    
    \label{tab:bottle_bowl}
\end{table}
 

==> taxpose/tables/exec-l2-dist-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.70 & 0.80 & 0.83 & 0.90 & 0.70 & 0.92 & 0.70 & 0.86 & 0.73 & 0.74 & 0.66 & 0.87 & 0.74 & 0.69 & 0.63 & 0.67 & 0.63 & 0.75 & 0.72 & 0.83 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.57 & 0.70 & 0.79 & 0.82 & 0.66 & 0.65 & 0.63 & 0.62 & 0.49 & 0.66 & 0.64 & 0.67 & 0.50 & 0.85 & 0.54 & 0.75 & 0.43 & 0.70 & 0.45 & 0.61 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.26 & 0.50 & 0.46 & 0.50 & 0.16 & 0.38 & 0.19 & 0.48 & 0.30 & 0.50 & 0.13 & 0.55 & 0.28 & 0.57 & 0.44 & 0.50 & 0.14 & 0.63 & 0.24 & 0.40 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.14 & 0.68 & 0.16 & 0.69 & 0.10 & 0.73 & 0.10 & 0.84 & 0.17 & 0.76 & \textbf{0.05} & 0.88 & 0.12 & 0.51 & 0.29 & 0.54 & 0.12 & 0.68 & 0.16 & 0.47 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.11} & \textbf{0.10} &\textbf{ 0.12 }& \textbf{0.09} & \textbf{0.02} & \textbf{0.04} & \textbf{0.06} & \textbf{0.08} & \textbf{0.15} & \textbf{0.11} & 0.05 & \textbf{0.05} & \textbf{0.12} & \textbf{0.08} & \textbf{0.28} & \textbf{0.26} & \textbf{0.10 }& \textbf{0.09} & \textbf{0.07} & \textbf{0.06} \\ \hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> taxpose/tables/exec-l2-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.70&	0.83&	0.70&	0.70&	0.73&	0.66&	0.74&	0.63&	0.63&	0.72\\
Goal-Cond E2E DAgger&0.61&0.79&0.66&0.63&0.49&0.64&0.80&0.64&0.43&0.45\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.26&0.46&0.16&0.19&0.30&0.13&0.28&0.44&0.14&0.24\\
% {Ours w/ Lear}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
{Goal-Cond Goal Flow}&0.14&0.16&0.06&0.16&0.15&0.02&0.05&0.24&0.22&0.09\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.11&0.12&0.02&0.06&0.15&0.05&0.12&0.28&0.10&0.07\\
\hline
\end{tabular}
}
\caption{Execution Normalized L2 Distance Metric Results ($\downarrow$): Normalized L2 distances to the ground truth goal position after rollouts. The lower the better.}
\label{tab:exec-l2-dist}
\end{table*}

==> taxpose/tables/exec-sr-rate-merged.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
\rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 0.02 & 0.01 & 0.03 & 0.00 & 0.10 & 0.05 & 0.03 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
\multicolumn{1}{|l|}{} & E2E DAgger & 0.03 & 0.00 & 0.00 & 0.00 & 0.10 & 0.00 & 0.10 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 0.15 & 0.13 & 0.03 & 0.03 & 0.63 & 0.60 & 0.13 & 0.13 & 0.03 & 0.00 & 0.25 & 0.25 & 0.10 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.15 & 0.15 \\
\multicolumn{1}{|l|}{} & Goal Flow & 0.64 & 0.05 & 0.73 & 0.00 & 0.75 & 0.10 & 0.73 & 0.00 & 0.50 & 0.00 & 0.80 & 0.00 & \textbf{0.65} & 0.10 & 0.35 & 0.10 & 0.70 & 0.10 & 0.55 & 0.05 \\ \hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{ACRONYM} & \textbf{0.78} & \textbf{0.81} & \textbf{0.78} & \textbf{0.78} & \textbf{0.98} & \textbf{1.00} & \textbf{0.88} & \textbf{1.00} & \textbf{0.70} & \textbf{0.73} & \textbf{1.00} & \textbf{1.00} & 0.65 & \textbf{0.65} & \textbf{0.55} & \textbf{0.45} & \textbf{0.73} & \textbf{0.88} & \textbf{0.80} & \textbf{0.80} \\ \hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> taxpose/tables/exec-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.02&	0.03&	0.10&	0.03&	0.00&	0.00&	0.00&	0.00&	0.00&	0.00\\
Goal-Cond E2E DAgger&0.03&0.00&0.10&0.10&0.00&0.00&0.00&0.00&0.03&0.00\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.15&0.025&0.63&0.13&0.03&0.25&0.10&0.00&0.05&0.15\\
{Goal-Cond Goal Flow}&0.60&0.63&0.73&0.73&0.48&0.85&0.65&0.37&0.48&0.50\\
% \textbf{Ours 2/ FCL Collision Checker}&0.68&0.78&0.77&0.75&0.55&0.93&0.75&0.35&0.70&0.55\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.78&0.78&0.98&0.88&0.70&1.00&0.65&0.55&0.73&0.80\\
\hline
\end{tabular}
}
\caption{Execution Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized L2 distance less than 0.1 \textbf{and} there is no collision in the entire rollout trajectory) of different objects' categories after rollouts. The higher the better.}
\label{tab:exec-sr}
\end{table*}

==> taxpose/tables/gi-Rt-error-gc.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \setlength\tabcolsep{.2em}
% \begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 40.45 & 0.75 & 37.82 & 0.82 & 38.17 & 0.81 & 37.15 & 0.65 & 44.84 & 0.68 & 32.52 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
% \multicolumn{1}{|l|}{} & E2E DAgger & 36.85 & 0.71 & 34.15 & 0.76 & 36.50 & 0.74 & 36.61 & 0.66 & 40.91 & 0.65 & 30.67 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 35.37 & 0.66 & 31.24 & 0.82 & 33.89 & 0.69 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
% \multicolumn{1}{|l|}{} & Goal Flow & 26.46 & 0.16 & 25.88 & 0.15 & 26.29 & 0.10 & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & 0.18 & 20.96 & 0.24 & 29.02 & 0.23 & 22.13 & 0.20 \\
% % \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \hline
% \multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \end{tabular}
% }
% \caption{Goal Inference Rotational and Translational Error Results. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). }
% \label{tab:gi-Rt}
% \end{table}
% \vspace{-25pt}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.26 & 0.73 & 37.82 & 0.82 & 37.15 & 0.65 & 44.84 & 0.68 & 30.69 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction_app} & 37.96 & 0.69 & 34.15 & 0.76 & 36.61 & 0.66 & 40.91 & 0.65 & 24.87 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW_app} & 35.95 & 0.67 & 31.24 & 0.82 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW_app} & 26.64 & 0.17 & 25.88 & \textbf{0.15} & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & \textbf{0.18} & 20.96 & \textbf{0.24} & 29.02 & 0.23 & 22.13 & 0.20  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & 6.64 & \textbf{0.16} & 6.85 & 0.16 & 2.05 & \textbf{0.10} & 3.87 & 0.12 & 4.04 & 0.08 & 12.71 & 0.31 & \textbf{6.87} & 0.37 & 5.89 & 0.13 & 14.93 & 0.18 \\ 
% \multicolumn{1}{|l|}{} & \textbf{TAX-Pose GC} & 7.74 & 0.17 & \textbf{4.43} &\textbf{0.13} & 3.27 & 0.13 & 4.16 & \textbf{0.12} & \textbf{3.3} & \textbf{0.08} & \textbf{10.76} & 0.26 & 7.36 & 0.30 & 6.28 & 0.14 & 22.37 & 0.21 \\ \hline

\multicolumn{1}{|l|}{} & \textbf{TAX-Pose GC} & \textbf{4.94} & \textbf{0.16} & \textbf{6.18} &0.16 & \textbf{1.75} & \textbf{0.10} & \textbf{2.94 }& \textbf{0.10} & \textbf{3.02} & \textbf{0.06} & \textbf{10.15} & 0.27 & 6.93 & 0.35 & \textbf{3.76} & \textbf{0.11} & \textbf{4.76} & \textbf{0.11} \\ \hline

\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$). Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt}
\end{table}
% \vspace{-25pt}

==> taxpose/tables/gi-Rt-error.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
% \setlength\tabcolsep{.2em}
% \begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 40.45 & 0.75 & 37.82 & 0.82 & 38.17 & 0.81 & 37.15 & 0.65 & 44.84 & 0.68 & 32.52 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
% \multicolumn{1}{|l|}{} & E2E DAgger & 36.85 & 0.71 & 34.15 & 0.76 & 36.50 & 0.74 & 36.61 & 0.66 & 40.91 & 0.65 & 30.67 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow & 35.37 & 0.66 & 31.24 & 0.82 & 33.89 & 0.69 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
% \multicolumn{1}{|l|}{} & Goal Flow & 26.46 & 0.16 & 25.88 & 0.15 & 26.29 & 0.10 & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & 0.18 & 20.96 & 0.24 & 29.02 & 0.23 & 22.13 & 0.20 \\
% % \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \hline
% \multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
% \end{tabular}
% }
% \caption{Goal Inference Rotational and Translational Error Results. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). }
% \label{tab:gi-Rt}
% \end{table}
% \vspace{-25pt}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
\begin{table}[h]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.26 & 0.73 & 37.82 & 0.82 & 37.15 & 0.65 & 44.84 & 0.68 & 30.69 & 1.06 & 40.38 & 0.69 & 45.09 & 0.76 & 45.00 & 0.79 & 45.65 & 0.64 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction} & 37.96 & 0.69 & 34.15 & 0.76 & 36.61 & 0.66 & 40.91 & 0.65 & 24.87 & 0.97 & 35.95 & 0.70 & 40.34 & 0.74 & 32.86 & 0.79 & 39.45 & 0.53 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW} & 35.95 & 0.67 & 31.24 & 0.82 & 39.21 & 0.72 & 34.35 & 0.66 & 28.48 & 0.75 & 37.14 & 0.59 & 29.49 & 0.70 & 39.60 & 0.76 & 39.69 & 0.48 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW} & 26.64 & 0.17 & 25.88 & \textbf{0.15} & 25.05 & 0.15 & 30.62 & 0.15 & 27.61 & 0.10 & 28.01 & \textbf{0.18} & 20.96 & \textbf{0.24} & 29.02 & 0.23 & 22.13 & 0.20  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.64} & \textbf{0.16} & \textbf{6.85} & 0.16 & \textbf{2.05} & \textbf{0.10} & \textbf{3.87} & \textbf{0.12} & \textbf{4.04} & \textbf{0.08} & \textbf{12.71} & 0.31 & \textbf{6.87} & 0.37 & \textbf{5.89} & \textbf{0.13} & \textbf{14.93} & \textbf{0.18} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$). Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt}
\end{table}
% \vspace{-25pt}

==> taxpose/tables/gi-chamfer-dist-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> taxpose/tables/gi-chamfer-dist.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.69&	0.77&	0.71&	0.72&	0.65&	0.70&	0.65&	0.64&	0.68&	0.67\\
Goal-Cond E2E DAgger&0.49&0.71&0.39&0.56&0.43&0.55&0.42&0.42&0.50&0.43\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.25&0.39&0.19&0.28&0.27&0.11&0.26&0.27&0.33&0.18\\
Goal-Cond Goal Flow&0.14&0.10&0.06&0.16&0.15&0.07&0.05&0.24&0.22&0.18\\
Goal-Cond DCP&0.54&0.66&0.47&0.70&0.28&0.45&0.78&0.32&0.67&0.50\\
Goal-Cond DCP Weighted Sum&0.37	&0.56&	0.19&	0.57&	0.35&	0.23&	0.56&	0.28&	0.48&	0.12\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.07&0.05&0.00&0.09&0.19&0.01&0.03&0.14&0.05&0.08\\
\hline
\end{tabular}
}
\caption{Goal Inference Normalized Chamfer Distance Metric Results ($\downarrow$): Normalized Chamfer distances to the point cloud under ground truth goal pose. The lower the better.}
\label{tab:gi-chamfer-dist}
\end{table*}

==> taxpose/tables/gi-sr-rate-merged.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.09 & 0.03 & 0.00 & 0.00 & 0.10 & 0.00 & 0.00 & 0.05 & 0.15 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.00 & 0.10 & 0.10 & 0.00 & 0.05 & 0.00 \\
\multicolumn{1}{|l|}{} &  E2E DAgger & 0.31 & 0.05 & 0.00 & 0.30 & 0.50 & 0.03 & 0.23 & 0.03 & 0.33 & 0.03 & 0.50 & 0.00 & 0.25 & 0.00 & 0.15 & 0.10 & 0.40 & 0.00 & 0.40 & 0.00 \\ \hline
\multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.61 & 0.39 & 0.28 & 0.13 & 0.75 & 0.50 & 0.53 & 0.50 & 0.50 & 0.15 & 0.80 & 0.75 & 0.80 & 0.20 & 0.55 & 0.50 & 0.50 & 0.25 & 0.75 & 0.50 \\
\multicolumn{1}{|l|}{} &  Goal Flow & 0.74 & 0.42 & 0.75 & 0.40 & 0.88 & 0.63 & 0.78 & 0.22 & \textbf{0.80} & 0.60 & 0.83 & 0.50 & 0.75 & 0.50 & 0.65 & 0.05 & 0.63 & 0.25 & 0.65 & 0.65 \\
\multicolumn{1}{|l|}{} &  Pose Match & 0.29 & 0.30 & 0.25 & 0.20 & 0.30 & 0.30 & 0.00 & 0.00 & 0.68 & 0.58 & 0.38 & 0.43 & 0.10 & 0.00 & 0.45 & 0.65 & 0.10 & 0.18 & 0.40 & 0.40 \\
\multicolumn{1}{|l|}{} &  Pose Match WS & 0.38 & 0.44 & 0.20 & 0.20 & 0.65 & 0.63 & 0.05 & 0.15 & 0.45 & 0.60 & 0.58 & 0.38 & 0.15 & 0.50 & 0.45 & 0.35 & 0.28 & 0.20 & 0.65 & 0.65 \\ \hline
\multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.90} & \textbf{0.88} & \textbf{0.93} & \textbf{0.88} & \textbf{1.00} & \textbf{0.98} & \textbf{0.85} & \textbf{0.95} & 0.80 & \textbf{0.70} & \textbf{1.00} & \textbf{1.00 }& \textbf{0.95} & \textbf{0.80} & \textbf{0.75} & \textbf{0.75} & \textbf{0.95 }& \textbf{0.93 }& \textbf{0.90} & \textbf{0.95} \\ \hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> taxpose/tables/gi-sr-rate.tex <==
\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|r|c|ccccccccc|}
 \hline
 \rule{0pt}{2.5em}
 & \textbf{\underline{AVG.}} &\clipart{microwave} &\clipart{chair}&\clipart{dishwasher}&\clipart{oven}&\clipart{fridge}&\clipart{table}&\clipart{washingmachine}&\clipart{safe}&\clipart{drawer}\\
\hline
 \textbf{Baselines} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond E2E BC&0.09&	0.00&	0.10&	0.00&	0.15&	0.25&	0.15&	0.00&	0.10&	0.05\\
Goal-Cond E2E DAgger&0.31&0.00&0.50&0.23&0.33&0.50&0.25&0.15&0.40&0.40\\
\hline
 \textbf{Ablations} & \multicolumn{10}{c|}{} \\
\hline
Goal-Cond Traj. Flow&0.61&0.28&0.75&0.53&0.50&0.80&0.80&0.55&0.50&0.75\\
{Goal-Cond Goal Flow}&0.74&0.75&0.88&0.78&0.80&0.83&0.75&0.65&0.625&0.65\\
Goal-Cond DCP&0.29&0.25&0.30&0.00&0.68&0.38&0.10&0.45&0.10&0.40\\
Goal-Cond DCP Weighted Sum&0.38&	0.20&	0.65&	0.05&	0.45&	0.58&	0.15&	0.45&	0.275&	0.65\\
\hline
 \textbf{Ours} & \multicolumn{10}{c|}{} \\
\hline
\textbf{Goal-Cond DCP + Res. Flow}&0.90&0.93&1.00&0.85&0.80&1.00&0.95&0.75&0.95&0.90\\
\hline
\end{tabular}
}
\caption{Goal Inference Success Rate Metric Results ($\uparrow$): Fraction of success trials (normalized Chamfer distance less than 0.1) of different objects' categories in goal inference only. The higher the better.}
\label{tab:gi-sr}
\end{table*}

==> taxpose/tables/gi_sim_Rt_goal0.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-20} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.37 & 0.69 & 40.49 & 0.80 & 50.79 & 0.59 & 48.02 & 0.61 & 30.69 & 1.09 & 36.59 & 0.81 & 48.48 & 0.42 & 41.42 & 0.84 & 42.49 & 0.37 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction_app} & 36.06 & 0.67 & 38.57 & 0.68 & 43.99 & 0.63 & 42.34 & 0.57 & 24.87 & 0.96 & 30.87 & 0.90 & 42.96 & 0.46 & 29.79 & 0.83 & 35.08 & 0.33 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW_app} & 34.48 & 0.65 & 35.39 & 0.85 & 43.42 & 0.63 & 35.51 & 0.60 & 28.26 & 0.80 & 27.67 & 0.68 & 25.91 & 0.44 & 43.59 & 0.82 & 36.05 & 0.36 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW_app} & 27.49 & \textbf{0.21} & 25.41 & \textbf{0.08} & 31.07 & 0.13 & 27.05 & 0.27 & 27.80 & 0.11 & 29.02 & \textbf{0.38} & 19.22 & \textbf{0.36} & 31.56 & 0.18 & \textbf{28.81} & \textbf{0.19} \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{11.74} & 0.23 & {\textbf{5.81}} & {0.11} & {\textbf{1.82}} & {\textbf{0.08}} & {\textbf{5.92}} & {\textbf{0.11}} & {\textbf{3.67}} & {\textbf{0.07}} & {\textbf{19.54}} & {0.41} & {\textbf{7.96}} & {0.63} & {\textbf{5.96}} & {\textbf{0.12}} & {43.27} & {0.33} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{In'}' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal0}
\end{table}

==> taxpose/tables/gi_sim_Rt_goal1.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-16} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 42.69 & 0.74 & 41.94 & 0.74 & 36.70 & 0.52 & 38.23 & 0.73 & 41.69 & 1.10 & 48.57 & 0.75 & 48.98 & 0.63 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction_app} & 37.68 & 0.70 & 39.24 & 0.69 & 31.63 & 0.54 & 41.06 & 0.68 & 37.72 & 1.03 & 35.94 & 0.75 & 40.47 & 0.51 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW_app} & 35.13 & 0.76 & 34.78 & 0.70 & 39.14 & 0.59 & 31.10 & 0.69 & 33.07 & 0.97 & 35.61 & 0.71 & 37.09 & 0.87 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW_app} & 22.10 & 0.20 & 27.82 & 0.26 & 20.43 & \textbf{0.09} & 34.66 & 0.10 & 22.71 & 0.12 & 26.48 & 0.27 & 0.48 & 0.32 \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{4.45} & \textbf{0.12} & \textbf{4.21} & \textbf{0.12} & \textbf{2.29} & 0.10 & \textbf{2.73} & \textbf{0.09} & \textbf{5.77} & \textbf{0.10} & \textbf{5.81} & \textbf{0.13} & \textbf{5.89} & \textbf{0.19} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{On}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal1}
\end{table}

==> taxpose/tables/gi_sim_Rt_goal2.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-16} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 44.87 & 0.74 & 30.95 & 0.89 & 36.86 & 0.72 & 56.86 & 0.52 & 34.35 & 1.03 & 31.69 & 0.77 & 46.86 & 0.78 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction_app} & 41.32 & 0.68 & 31.40 & 0.84 & 38.49 & 0.73 & 47.64 & 0.51 & 36.47 & 0.99 & 27.72 & 0.73 & 39.83 & 0.51 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW_app} & 38.85 & 0.58 & 31.87 & 1.07 & 39.48 & 0.44 & 39.48 & 0.44 & 28.71 & 0.69 & 41.06 & 0.73 & 40.70 & 0.31 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW_app} & 29.64 & \textbf{0.10} & 28.51 & \textbf{0.10} & 26.33 & \textbf{0.08} & 32.96 & \textbf{0.07} & 27.42 & 0.10 & 22.04 & \textbf{0.09} & 27.42 & 0.15  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{6.02} & 0.17 & \textbf{12.73} & 0.28 & \textbf{1.59} & 0.11 & \textbf{2.91} & 0.12 & \textbf{4.41} & \textbf{0.08} & \textbf{12.12} & 0.34 & \textbf{6.38} & \textbf{0.12} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{Left}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal2}
\end{table}

==> taxpose/tables/gi_sim_Rt_goal3.tex <==
\begin{table}[H]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|lr|cc|cc|cc|cc|cc|cc|}
\hline
 \rule{0pt}{2.5em}
 & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} &  \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-14} 
 & \multicolumn{1}{l|}{} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} & \textbf{$\mathcal{E}_\mathbf{R}$} & \textbf{$\mathcal{E}_\mathbf{t}$} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Baselines}}} & E2E BC & 39.11 & 0.76 & 37.89 & 0.86 & 24.26 & 0.77 & 36.27 & 0.88 & 52.86 & 0.48 & 44.26 & 0.78 \\
\multicolumn{1}{|l|}{} & E2E DAgger~\cite{ross2011reduction_app} & 36.80 & 0.73 & 27.40 & 0.84 & 32.31 & 0.74 & 32.61 & 0.82 & 49.27 & 0.46 & 42.40 & 0.78 \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{Ablations}}} & Traj. Flow~\cite{EisnerZhang2022FLOW_app} & 35.33 & 0.71 & 22.93 & 0.66 & 34.78 & 1.22 & 31.29 & 0.92 & 42.71 & 0.37 & 44.93 & 0.36 \\
\multicolumn{1}{|l|}{} & Goal Flow~\cite{EisnerZhang2022FLOW_app} & 27.34 & 0.16 & 21.79 & 0.15 & 22.37 & 0.28 & 27.79 & 0.15 & 32.96 & \textbf{0.07} & 31.79 & 0.15  \\
% \multicolumn{1}{|l|}{} & CPE Only & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
\hline
\multicolumn{1}{|l|}{\textbf{Ours}} & \textbf{TAX-Pose} & \textbf{4.33} & \textbf{0.13} & \textbf{4.64} & \textbf{0.14} & \textbf{2.48} & \textbf{0.11} & \textbf{3.91} & \textbf{0.15} & \textbf{6.47} & 0.17 & \textbf{4.17} & \textbf{0.08} \\ \hline
\end{tabular}
}
\caption{Goal Inference Rotational and Translational Error Results ($\downarrow$) for the ``\textbf{Right}'' Goal. Rotational errors ($\mathcal{E}_\mathbf{R}$) are in degrees ($^\circ$) and translational errors ($\mathcal{E}_\mathbf{t}$) are in meters ($\mathrm{m}$). The lower the better.}
\label{tab:gi-Rt_goal3}
\end{table}

==> taxpose/tables/mug_hanging_exp_main.tex <==
    \noindent \begin{minipage}[t]{.4\textwidth}
    \label{tab:mug_on_rack_few_shot}
    % \small
        \centering
        \begin{tabular}{c|c c c}
            \hline
            \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
            \hline
            & 1 & 5 & 10\\
            \hline
            DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
            NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
            \textbf{TAX-Pose (Ours)} & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
            \hline
        \end{tabular}
        \captionof{table}{ \# Demos vs. Overall Success}

    \end{minipage}%
    \qquad\qquad
    \begin{minipage}[t]{.5\textwidth}
        % \small
        \centering
        \label{tab:mug_resul}
  \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
        \captionof{table}{Mug Hanging Ablations Results}

    \end{minipage}%
    
    \begin{table}[h]
    % \small
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    }
    \caption{Mug on Rack Simulation Task Success Results
    % \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
    }
    \label{tab:mug_on_rack_exp}
\end{table}

==> taxpose/tables/mug_on_rack_exp.tex <==
\begin{table}[h]
    % \small
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c|c c c| c c c}
    \hline
     & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
    % & Grasp & Place & Overall\\
    \hline
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
     &\multicolumn{3}{c|}{\textbf{Upright Pose}}& \multicolumn{3}{c}{\textbf{Arbitrary Pose}} \\
         \hline
         DON \cite{florence2018dense} & 0.91 &0.50 & 0.45 & 0.35 & 0.45& 0.17 \\
         NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88  & \textbf{0.78} &0.75 & 0.58\\
         \textbf{TAX-Pose (Ours)} & \textbf{0.99}& \textbf{0.97}& \textbf{0.96} &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    \hline
        %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

    % \textbf{Arbitrary Pose} & & & \\
    %  \hline
    %      DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
    %      NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
    %       TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
    % \hline
    \end{tabular}
    }
    \caption{Mug on Rack Simulation Task Success Results
    % \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
    }
    \label{tab:mug_on_rack_exp}
\end{table}
% \vspace{-1em}
% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%      & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
%     % & Grasp & Place & Overall\\
%     \hline
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
%     \hline
%         \textbf{Upright Pose} & & &\\
%          \hline
%          DON \cite{florence2018dense} & 0.91 &0.50 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.96 & 0.92 & 0.88 \\
%          TAX-Pose (Ours) & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%         %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 5^{\circ}$}}\\

%     \textbf{Arbitrary Pose} & & & \\
%      \hline
%          DON \cite{florence2018dense} & 0.35 & 0.45& 0.17 \\
%          NDF \cite{simeonov2021neural} & \textbf{0.78} &0.75 & 0.58\\
%           TAX-Pose (Ours)  &  0.75& \textbf{0.84}& \textbf{0.63}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug on Rack Simulation Task Success Results
%     \dave{Let's make this table horizontal to save space (put ``arbitrary pose" to the right of upright pose) - OR wrap text around it}
%     }
 
%     \label{tab:mug_on_rack_exp}
% \end{table}

==> taxpose/tables/mug_on_rack_few_shot.tex <==
% \begin{table}[h]
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%       \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
%         \end{adjustbox}
%     %\caption{Mug on Rack Simulation Task Success Results with Varying Number of Demo Used
%     %\dave{Too much whitespace around this table; wrap text around it}
%     %}
 
%     %  \label{tab:mug_on_rack_few_shot}
     
%  \end{subtable}

% % \hfill
% \begin{subtable}[h]{0.1\textwidth}
%     \centering
%      \begin{adjustbox}{0.2\textwidth}
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
     
%     \end{tabular}
%     \end{adjustbox}

 
%   #%\label{tab:mug_rack_ablation}
%  \end{subtable}
%     \caption{Mug on Rack Ablation  Results}
%     \label{tab:mug_rack_ablation}
% \end{table}


%  \begin{table}[h]
 
%     \centering
     
%     \begin{tabular}{c|c c c}
%     % \hline
%      \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
%     \hline
 
    
%     \end{tabular}
        
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
%     % \dave{Too much whitespace around this table; wrap text around it}
%     }
 
%      \label{tab:mug_on_rack_few_shot}
     
%  \end{table}


% \begin{table}[h]
% \begin{varwidth}[b]{0.33\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
%     \hline
%           & 1 & 5 & 10\\
%          \hline
%          DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
%          NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
%           TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
%     \hline
%     \end{tabular}
%     \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success}
%      \label{tab:mug_on_rack_few_shot}
% \end{varwidth}%
% \begin{varwidth}[b]{0.2\linewidth}
%     \centering
%     \begin{tabular}{c|c c c}
%     \hline
%     \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
%          No Residual Correspondence  & 0.97 &0.96 & 0.93\\
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
%          3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
%          TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
%     \hline
%     \end{tabular}
%     \caption{Mug Hanging Ablations Results}
%     \label{tab:mug_rack_ablation}
% \end{varwidth}%

% \end{table}

 
 \begin{wraptable}{r}{8cm}
 
    \centering
     
    \begin{tabular}{c|c c c}
    % \hline
     \textbf{Model} & \multicolumn{3}{c} \#\textbf{Demos Used }\\
    \hline
          & 1 & 5 & 10\\
         \hline
         DON \cite{florence2018dense}  & 0.32 &0.36 & 0.45\\
         NDF \cite{simeonov2021neural} &  0.46 & 0.70 & 0.88 \\
          TAX-Pose (Ours) & \textbf{0.77}& \textbf{0.90}& \textbf{0.96}\\
         
    \hline
 
    
    \end{tabular}
        
    \caption{Analysis of Number of Demonstrations Used in Training on Upright Pose Mug Hanging Task Success
    % \dave{Too much whitespace around this table; wrap text around it}
    }
 
     \label{tab:mug_on_rack_few_shot}
     
 \end{wraptable}
 

==> taxpose/tables/mug_rack_ablation.tex <==
% \begin{table}[h]
\begin{table}[]
  \tiny
    \centering
    \begin{tabular}{c|c c c}
    \hline
    \textbf{Ablation} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
         No Residual Correspondence  & 0.97 &0.96 & 0.93\\
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
         3-Layer MLP In Place of Attention &  0.90 & 0.82 & 0.76 \\
         TAX-Pose (Ours)  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\
         
    \hline
    \end{tabular}
    \caption{Mug Hanging Ablations Results}
    \label{tab:mug_rack_ablation}
\end{table}



 

==> taxpose/tables/mug_rack_ablation_large_scale.tex <==
% % \begin{table}[h]
% \begin{table}[H]
 
%     \centering
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|c| c c c}
%     \hline
%   \textbf{Ablation Category} & \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
%     %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
%         % \textbf{Upright Pose} & & &\\
%          \hline
     
%          \multirow{4}{*}{\textit{Loss}}  & No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
%          & No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
%          & No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
%          & Scaled Combination of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ ($ 1.1*\mathcal{L}_\mathrm{cons} + 1*\mathcal{L}_\mathrm{corr}$) &  0.10 & 0.01 & 0.01 \\
%          \hline 
%          \multirow{1}{*}{\textit{Residual Correspondence}}  & No Residual Correspondence  & 0.97 &0.96 & 0.93\\
         
%          \hline 
%          \multirow{1}{*}{\textit{Weighted SVD}} & 
%          Unweighted SVD &  0.92 & 0.94 & 0.88 \\
         
%         \hline 
%         \multirow{2}{*}{\textit{Pretraining Embedding Network}} &
     
%          No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
%          & No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         
%          \hline 
%         \multirow{1}{*}{\textit{Architecture for Cross-Object Attention}} & 
%          3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
         
         
%         \hline
%       \multirow{1}{*}{\textit{\# Dimensions for Embedding}} &
%         Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
%         \hline
%         \hline
%         \textbf{\textit{Ours}} & \textbf{TAX-Pose}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\

         
%     \hline
%     \end{tabular}
%     }
%     \caption{Mug Hanging Ablations Results Full Scale}
%     \label{tab:mug_rack_ablation_full}
% \end{table}



 % \begin{table}[h]
\begin{table}[H]
 
    \centering
\renewcommand{\arraystretch}{1.2}  % good vertical spacing for the long text descriptions.
\resizebox{0.85\textwidth}{!}{
    \begin{tabular}{c| c c c}
    \hline
  \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall}\\
  
    %  & \multicolumn{3}{c}{\textit{Avg Pairwise Angular Error $< 1^{\circ}$}}\\
   
        % \textbf{Upright Pose} & & &\\
         \hline
        % \textit{Loss}&&&\\
          No $\mathcal{L}_\mathrm{disp}$ &  0.01 & 0 & 0 \\
          No $ \mathcal{L}_\mathrm{corr}$ &  0.89 & 0.91 & 0.84 \\
           No $  \mathcal{L}_\mathrm{cons}$ &  \textbf{0.99} & 0.95 & 0.94 \\
            Scaled Combination: 
            %of  $ \mathcal{L}_\mathrm{corr} \&   \mathcal{L}_\mathrm{cons}$ (
            $ 1.1\mathcal{L}_\mathrm{cons} + \mathcal{L}_\mathrm{corr}$ &  0.10 & 0.01 & 0.01 \\
         \hline 
          No Adjustment via Correspondence Residuals  & 0.97 &0.96 & 0.93\\
         \hline 
         Unweighted SVD &  0.92 & 0.94 & 0.88 \\
        \hline 
         No Finetuning for Embedding Network &  0.98 & 0.93 & 0.91 \\
         No Pretraining for Embedding Network &  \textbf{0.99} & 0.72 & 0.71 \\
         \hline 
         3-Layer MLP In Place of Transformer &  0.90 & 0.82 & 0.76 \\
        \hline
        Embedding Network Feature Dim = 16 & 0.98 & 0.59 & 0.57 \\
    
        \hline
        \hline
        \textbf{TAX-Pose (Ours)}  & \textbf{0.99}& \textbf{0.97}& \textbf{0.96}\\

         
    \hline
    \end{tabular}
    }
    \caption{Mug Hanging Ablations Results}
    \label{tab:mug_rack_ablation_full}
\end{table}



 

==> taxpose/tables/no_pretraining.tex <==

\begin{table}[H]
 
    \centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
    \begin{tabular}{c| c c c|c c}
    \hline
  \textbf{Ablation Experiment} & \textbf{Grasp} & \textbf{Place} & \textbf{Overall} & \textbf{Train Rotation Error} & \textbf{Train Translation Error}  \\
   &   &   &   & \textbf{ (${}^{\circ}$)} & \textbf{(m)}  \\
  \hline
   \hline
  
         No Pre-Training for Embedding Network &  \multirow{2}{*}{\textbf{0.99}} &\multirow{2}{*}{ 0.92} & \multirow{2}{*}{0.92} & \multirow{2}{*}{4.91} & \multirow{2}{*}{\textbf{0.01}} \\ 
         (trained for 26K steps) &   &  &  &   & \\ 
         \hline 
        No Pre-training for Embedding Network &  \multirow{2}{*}{\textbf{0.99}} &\multirow{2}{*}{0.72} & \multirow{2}{*}{0.71} & \multirow{2}{*}{15.39} & \multirow{2}{*}{\textbf{ 0.01}} \\
          (trained for 15K steps) &   &  &  &  & \\ 
     
         \hline
        \textbf{TAX-Pose (Ours)} &  \multirow{2}{*}{\textbf{0.99}} &\multirow{2}{*}{\textbf{0.97}} & \multirow{2}{*}{\textbf{0.96}} & \multirow{2}{*}{\textbf{4.33}} & \multirow{2}{*}{\textbf{ 0.01}} \\ 
         (trained for 15K steps) &   &  &  &  & \\ 
    \hline
    \end{tabular}
    }
    \caption{Ablation Experiments on the Effects of Pre-Training. We report the task success rate for upright mug hanging task over 100 trials each, as well as the grasping model's training rotational error (${}^{\circ}$) and translation error (m).}
    \label{tab:no_pretraining_longer}
\end{table}



==> taxpose/tables/rw-placement.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
% \centering
% \begin{tabular}{|r|c|c|c|c|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\textbf{AVG. SR}} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
% Goal Flow & 0.31 & 0.18 & 0.38 & 0.37 \\ \hline
% \textbf{TAX-Pose} & 0.92 & 0.95 & 0.95 & 0.85 \\ \hline
% \end{tabular}
\begin{tabular}{|r|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \multicolumn{1}{l|}{\clipart{oven}} \\ \hline
Goal Flow & 0.18 & 0.38 & 0.37 \\ \hline
\textbf{TAX-Pose} & 0.95 & 0.95 & 0.85 \\ \hline
\end{tabular}
\label{rw-placement}
\caption{PartNet-Mobility Objects Placement Task Real-World Results.}
\end{table}

==> taxpose/tables/rw_each.tex <==
\begin{table}[H]
\renewcommand{\arraystretch}{1.2}
\resizebox{0.6\textwidth}{!}{
\setlength\tabcolsep{.2em}
\begin{tabular}{|l|lll|lll|lll|}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c|}{\textbf{In}} & \multicolumn{3}{c|}{\textbf{On}} & \multicolumn{3}{c|}{\textbf{Left}} \\ \cline{2-10} 
 & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} & \multicolumn{1}{l|}{\clipart{drawer}} & \multicolumn{1}{l|}{\clipart{fridge}} & \clipart{oven} \\ \hline
Goal Flow & \multicolumn{1}{l|}{0.00} & \multicolumn{1}{l|}{0.10} & 0.30 & \multicolumn{1}{l|}{0.05} & \multicolumn{1}{l|}{N/A} & 0.20 & \multicolumn{1}{l|}{0.50} & \multicolumn{1}{l|}{0.65} & 0.60 \\
\textbf{TAX-Pose} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{\textbf{1.00}} & \textbf{0.85} & \multicolumn{1}{l|}{\textbf{1.00}} & \multicolumn{1}{l|}{N/A} & \textbf{1.00} & \multicolumn{1}{l|}{\textbf{0.85}} & \multicolumn{1}{l|}{\textbf{0.90}} & \textbf{0.70} \\ \hline
\end{tabular}
}
\caption{Combined per-task results for real-world goal placement success rate.}
\label{tab:rw_each}
\end{table}

==> taxpose/tables/single_goal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h]
\begin{subtable}[h]{\textwidth}
    \centering
    \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
    \hline
    \rule{0pt}{2.5em}
    
    & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
    
    & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
    
    \end{tabular}
    \caption{First Week}
    \label{tab:week1}
\end{subtable}
\begin{subtable}[h]{\textwidth}
        \centering
        \begin{tabular}{l | l | l}
        Day & Max Temp & Min Temp \\
        \hline \hline
        Mon & 20 & 13\\
        Tue & 22 & 14\\
        Wed & 23 & 12\\
        Thurs & 25 & 13\\
        Fri & 18 & 7\\
        Sat & 15 & 13\\
        Sun & 20 & 13
       \end{tabular}
      \caption{First Week}
       \label{tab:week2}
\end{subtable}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|lr|rl|ll|ll|ll|ll|ll|ll|ll|ll|ll|}
% \hline
%  \rule{0pt}{2.5em}
%  & \multicolumn{1}{l|}{} & \multicolumn{2}{c|}{{ \textbf{AVG.}}} & \multicolumn{2}{c|}{\clipart{microwave}} & \multicolumn{2}{c|}{\clipart{chair}} & \multicolumn{2}{c|}{\clipart{dishwasher}} & \multicolumn{2}{c|}{\clipart{oven}} & \multicolumn{2}{c|}{\clipart{fridge}} & \multicolumn{2}{c|}{\clipart{table}} & \multicolumn{2}{c|}{\clipart{washingmachine}} & \multicolumn{2}{c|}{\clipart{safe}} & \multicolumn{2}{c|}{\clipart{drawer}} \\ \cline{3-22} 
%  & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} & \multicolumn{1}{c}{\textbf{In}} & \multicolumn{1}{c|}{\textbf{Out}} \\ \hline
% \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{\scriptsize Baselines}}} &  E2E BC & 0.69 & 0.81 & 0.77 & 0.81 & 0.71 & 0.88 & 0.72 & 0.86 & 0.65 & 0.79 & 0.70 & 0.68 & 0.65 & 0.69 & 0.64 & 0.69 & 0.68 & 0.79 & 0.67 & 0.88 \\
% \multicolumn{1}{|l|}{} &  E2E DAgger & 0.49 & 0.68 & 0.71 & 0.79 & 0.39 & 0.69 & 0.56 & 0.60 & 0.43 & 0.60 & 0.55 & 0.91 & 0.42 & 0.84 & 0.42 & 0.67 & 0.50 & 0.63 & 0.43 & 0.58 \\ \hline
% \multicolumn{1}{|l|}{\multirow{4}{*}{\textbf{\scriptsize Ablations}}} &  Traj. Flow & 0.25 & 0.49 & 0.39 & 0.54 & 0.19 & 0.42 & 0.28 & 0.53 & 0.27 & 0.53 & 0.11 & 0.62 & 0.26 & 0.32 & 0.27 & 0.42 & 0.33 & 0.58 & 0.18 & 0.45 \\
% \multicolumn{1}{|l|}{} &  Goal Flow & 0.14 & 0.37 & 0.10 & 0.36 & 0.06 & 0.35 & 0.16 & 0.52 & \textbf{0.15} & 0.25 & 0.07 & 0.34 & 0.05 & 0.40 & 0.24 & 0.45 & 0.22 & 0.50 & 0.18 & 0.13 \\
% \multicolumn{1}{|l|}{} &  Pose Match & 0.54 & 0.53 & 0.66 & 0.66 & 0.47 & 0.48 & 0.70 & 0.69 & 0.28 & 0.29 & 0.45 & 0.43 & 0.78 & 0.73 & 0.32 & 0.33 & 0.67 & 0.68 & 0.50 & 0.44 \\
% \multicolumn{1}{|l|}{} &  Pose Match WS & 0.37 & 0.36 & 0.56 & 0.54 & 0.19 & 0.18 & 0.57 & 0.53 & 0.35 & 0.28 & 0.23 & 0.18 & 0.56 & 0.33 & 0.28 & 0.41 & 0.48 & 0.54 & 0.12 & 0.22 \\ \hline
% \multicolumn{1}{|l|}{\textbf{\scriptsize Ours}} &  \textbf{ACRONYM} & \textbf{0.07} & \textbf{0.08} & \textbf{0.05} & \textbf{0.08} & \textbf{0.00} & \textbf{0.02} & \textbf{0.09} & \textbf{0.05} & 0.19 & \textbf{0.21 }& \textbf{0.01} & \textbf{0.02} & \textbf{0.03} &\textbf{ 0.11} & \textbf{0.14} & \textbf{0.14} &\textbf{ 0.05} & \textbf{0.08 }& \textbf{0.08} & \textbf{0.03} \\ \hline
% \end{tabular}
% }
\caption{Ben testing something o}
\label{tab:single-goal}
\end{table}
